ConcurORAM: High-Throughput Stateless Parallel Multi-Client ORAM

ConcurORAM is a parallel, multi-client oblivious RAM (ORAM) that eliminates waiting for concurrent stateless clients and allows overall throughput to scale gracefully, without requiring trusted third party components (proxies) or direct inter-client coordination. A key insight behind ConcurORAM is the fact that, during multi-client data access, only a subset of the concurrently-accessed server-hosted data structures require access privacy guarantees. Everything else can be safely implemented as oblivious data structures that are later synced securely and efficiently during an ORAM "eviction". Further, since a major contributor to latency is the eviction - in which client-resident data is reshuffled and reinserted back encrypted into the main server database - ConcurORAM also enables multiple concurrent clients to evict asynchronously, in parallel (without compromising consistency), and in the background without having to block ongoing queries. As a result, throughput scales well with increasing number of concurrent clients and is not significantly impacted by evictions. For example, about 65 queries per second can be executed in parallel by 30 concurrent clients, a 2x speedup over the state-of-the-art. The query access time for individual clients increases by only 2x when compared to a single-client deployment.

==> analysis.tex <==
\section{Extensions}
\label{analysis}
%


{\color{blue}



\subsection{Fault Tolerance}
%
In general, achieving fault tolerance for ORAMs in a distributed setting is challenging, as clients share responsibilities without explicit interaction. In the following, we discuss protocols that allow \sysname~ to proceed gracefully in the event of system crashes, network failures etc.


\smallskip
\noindent
{\bf Crashes during queries.~} The query stages where a client can fail are listed below --

\begin{enumerate}
	\item {\em Updating the query log (Algorithm \ref{query}, Steps 1 - 4):} If the client fails while updating the query log, it will do so while holding the query lock. In this case after a specified timeout, the other concurrent clients can simply proceed with their queries. 
	\item {\em Prior to adding queried block to DRL (Algorithm \ref{query}, Steps 5 - 12):} In this case, the client has not yet updated the current data result log with the result of its query. Recall that clients that started execution later wait for this result. After a specified timeout, the {\em next} client waiting for access to the data result log can repeat the query on behalf of the failed client and add the result to the data result log. 
	
	Observe that this does not leak privacy -- if a query fails, the {\em next} client (public information),  always repeats the query after a specified time, regardless of this client's own query, resulting in exactly the same access pattern. 
	
	\item {\em Reshuffling the bigentry log and temporary stashes:} In this case, the failed client will not write back to the temporary workspace. The client that replaces the old versions with the reshuffled version at the end of a query round, can perform the required reshuffles without any additional assistance.
\end{enumerate}	


\smallskip
\noindent
{\bf Crashes during evictions.~} Evictions can fail at various stages, and although specified timeouts will allow the protocol to proceed, it is important to know whether to {\em roll back} changes and start afresh, or to {\em roll through} and continue with the protocol for the sake of consistency. 

\begin{itemize} 
	\item {\em Stage 1:} If the eviction fails in stage 1, which only includes read-only access to the write-only tree, a different client can takeover and start afresh.
	
	\item {\em Stage 2 (critical section):} In stage 2, the eviction will fail while holding the {\em processing lock}. As a result, subsequent evictions waiting for results from the critical section will not proceed. In case of a crash, the eviction can be restarted by another client after rolling back the changes performed in the critical section. Effectively this means disregarding any changes made in the critical section (to the EST buckets and temporary stash) by the failed client and starting afresh.
	
	\item {\em Stage 3:} At this stage, results generated in the critical section by the failed evictions may have been used by subsequent evictions entering the critical section. Thus, the changes cannot be rolled-back. Instead, a different client can continue with the eviction process. This requires one critical piece of information -- {\em the pseudo-random mapping} used by the failed eviction for mapping blocks in the bigentry logs to new paths in the data tree. While in the critical section, this information is added to the {\em eviction log}, and can be used later by a different client for completing the eviction. 
	
	\item {\em Commits:} If the client fails during commits, a different client can perform the commit on its behalf, with some additional information -- 
	
	\begin{itemize}
		\item {\em Server-side cache} -- Firstly, all contents of the client-side cache which include the temporary stash and the eviction sub-tree buckets needs to be stored on the server. This can be used by a different client for committing updates, in case of a crash.
		
		\item {\em Eviction metadata.~} Additionally, the client that performs the eviction on behalf of the failed client has to perform several other tasks (as per the commit protocol in Section \ref{overview:non_blocking}). This includes -- i) updating the position map for blocks evicted, ii)  updating metadata on data tree path, and iii) clearing query log and data result log.
		

		To perform these tasks, the client requires the following additional {\em metadata}, which can be stored in the {\em eviction log} while in the critical section -- i) eviction identifier, ii) the identifier for the eviction path, iii) 
		The logical identifiers of the evicted blocks {\em and} the paths to which they are mapped in the data tree, and iv) the identifiers for the query log and the data result log.  
		
	\end{itemize}
\end{itemize}	



\subsection{Malicious Security}
%
Although the \sysname~ protocols are designed for an honest-but-curious server, security against a malicious server is desirable. In the following, we discuss how the \sysname~ protocols can be modified for a malicious server setting.

This is specially challenging since the clients do not communicate, which leaves open the possibility of server-mounted {\em replay attacks}. The strongest form of consistency achievable in this setting is {\em fork consistency} \cite{sundr} -- if the server selectively replays the states of server-side data structures and presents different (possibly conflicting) views of the system to different clients, then these views cannot be unified later without being detected.  

As a first step, integrity of the server-side data structures can be provided using existing techniques e.g., {\em embedding a Merkle tree in the ORAM tree} \cite{pathoram}, storing HMACs over the DR-LogSet, StashSet etc. In single client settings, the root of the Merkle tree and the HMACs can be cached client side and verified for each access. Unfortunately, in a multi-client setting, storing these on the server does not solve the problem due to replay attacks. Instead, we use this for achieving fork consistency.


%\medskip
%\noindent
%{\bf Integrity of data structures.~} 
%%
%In fact, notwithstanding replay attacks, an actively malicious server could simply overwrite data and violate integrity of the \sysname~ data structures, namely the data tree, the write-only tree, the DR-LogSet and the StashSet. Possible mitigations are listed below --
%
%
%\begin{itemize}
%	\item {\em Embedding a Merkle tree in data tree and write-only tree:} A standard technique for ensuring integrity of tree based ORAMs  is {\em embedding a Merkle tree in the ORAM tree} \cite{pathoram}. The Merkle tree can be updated as part of the evictions with negligible additional costs.
%	
%	This can be applied for the both the data tree and the write-only tree in \sysname~.  The embedded Merkle tree is updated as part of the evictions -- the data tree is updated during the commits, while the write-only tree is updated during the eviction processing.
%	
%	\item {\em HMACs over DR-LogSet and StashSet:} To protect integrity of the DR-LogSet and StashSet, {\em one possible solution is to store a HMAC over the concatenation of constituent blocks.} The HMACs are updated when the DR-LogSet and StashSet are updated with new reshuffled versions as part of the queries (Algorithm \ref{query}, Steps 15 - 17). Recall that periodic shuffles of the bigentry logs and temporary stashes is necessary to ensure that {\em unique} blocks are read for each query.
%\end{itemize}	




\smallskip
\noindent
{\bf Replay attacks on queries.~}
%
First, observe that a malicious server could mount several types of replay attacks in order to leak inter-client privacy --

\begin{enumerate}
	\item {\em Replaying the query log:} As pointed out by previous work \cite{privatefs}, the server could simply replay the query log, presenting different views of ongoing transactions to concurrent clients. As a result, clients querying for the same block will have the same resulting access pattern to the server data structures, leaking inter-client privacy. 	
	
	\item {\em Replaying data structure states:} The server could replay contents of the server-side data structure along with the Merkle tree root hashes, HMACs etc.
	
%	\item{\em Replaying counter values:} \sysname~ stores several server-side counters such as the processing counter, commit counter etc to provide global synchronization of evictions and queries without inter-client communication. The server can replay the values in order to leak inter-client privacy or/and cause inconsistencies in the system.
%	
\end{enumerate}
	
	
	 
\smallskip
\noindent
{\bf Fork consistency for queries.~}
%
Similar to previous work \cite{privatefs}, the key idea is to store a hash tree over all previous queries on the server. In addition, each client stores its own {\em last} query information locally. As part of each query, the client first verifies that the hash tree records its last query. If the server forks client views, updates to the hash tree by a particular client will need to be hidden from the other clients. As a result, the corresponding clients will see different updates to the hash tree (and resulting root hash values), for all subsequent queries. Moreover, if the clients interact at some point of time in the future and compare root hash values, the forking attack will be discovered

\smallskip
\noindent
{\em Protecting against query log replays:} We extend the idea here to prevent the replay attacks described above. Specifically, for each query, a client updates the hash tree with a new leaf record, which includes the following -- 

\begin{enumerate}
	\item The clients' own unique identifier
	\item The logical address of the block queried
\end{enumerate}	

This record is stored client side and as part of its {\em next} query, the client verifies that the record exists in the hash tree.  The intuition here is that since hashes are unforgeable, the server cannot add a new record to the hash tree and forge the root hash value in case of forking attacks. Further, the client's unique identifiers being included in the record ensures that even if two clients query for the same block, or update the same data structure contents (as a result of a forking attack), the hash records they generate will be different with very high probability, subject to a hashing function with high-collision resistance.


%\medskip
%\noindent
%{\em Correctness.~}
%%



\smallskip
\noindent
{\em Protecting against data structure replays:} Similarly, to protect against replay of data structure states, \sysname~ maintains a hash tree on the server recording the {\em data structure integrity variables}. Specifically, when the data tree, DR-LogSet or StashSet is updated, a leaf record is added to the tree with the new state variables that includes -- 

\begin{enumerate}
\item Updating client's identifier
\item Merkle tree root hash for the data tree
\item HMAC over DR-LogSet blocks
\item HMAC over the StashSet blocks
\end{enumerate}	 

The client that performs the updates stores the record locally and verifies that the record exists in the hash tree for subsequent accesses.  As updates to the DR-LogSet, StashSet and server-side trees are recorded by the hash tree, a client can verify their integrity while accessing them. If the server replays states, the client which performed the last update will have a different view of the data structures (root hashes, HMAC values) compared the other clients in the system. Thus, if the clients interact at some point of time in the future, the forking attack will be detected.



%\medskip
%\noindent
%{\em Correctness.~}
%%

%\smallskip
%\noindent
%{\bf Faulty locking.~}
%%
%The malicious server may not enforce proper locking which will result in inconsistencies  during evictions. This is similar to the server performing a {\em denial of service} attack by changing/deleting encrypted data. Subsequently, the inconsistencies will violate the tree-based ORAM invariants, and will be detected.
%}


==> construction.tex <==
\section{Putting It All Together}
\label{oram:final}
%
The synchronization of PD-ORAM (for storing position map entries) and
RingORAM (for storing data blocks) is critical for the security and performance of \sysname~.  In this
section, we discuss the parameters for \sysname~ and security for
multi-client concurrency.

\medskip
\noindent
{\bf Eviction Period.~} 
%
The eviction period, $e$
determines the number of concurrent accesses that can
be performed before an eviction.
Setting a higher eviction period increases the size of the
stash and the logs that need to be read by the client for an access. 
Further, RingORAM \cite{ringoram} provides theoretical bounds on the stash
for a given eviction period and experimentally verifies the same. 
More specifically, the bound on the stash is provided as a function of the 
bucket size and the eviction period. 
\sysname~ uses the empirical results from \cite{ringoram} to determine an
appropriate eviction period to bound the stash size to size $\order{logN}$. 

\medskip
\noindent
{\bf Stash Size.~}
%
\sysname~ ensures that the stash always contains the same number of entries 
irrespective of the 
outcome of an eviction. More specifically, if the number of blocks in the stash 
after an eviction is 
less than the total size of the stash, \sysname~ adds fake blocks to the empty 
locations.


\medskip
\noindent
{\bf PD-ORAM Bucket Size.~} 
% 
Recall that after an eviction, the entries from the PM result log 
form the top level of PD-ORAM. Consequently, the top level should 
hold at least as many entries as the PM result log. \sysname~ 
sets the size of the top level equal to the eviction period,$e$. Each bucket in the the following 
levels contains $e$ real entries and the bucket size is set to $\delta = e \times logN$ to 
handle hash collisions~\cite{privatefs}.

\medskip
\noindent
{\bf Query overhead for position map entry.~}
%
Note that a bucket with $c \times logN$ position map entries, each of size 
$\order{logN}$ is roughly equal to the size of a RingORAM data block. For 
e.g. 
for a 1TB database, with 20 clients and 8 byte position map entries, the size 
of 
a bucket is 4KB. Further, this implies that 
the bandwidth overhead for querying for the position map entry in PD-ORAM 
for a particular ORAM data block is equivalent to reading $\order{logN}$ data 
blocks. 
Recall that the amortized bandwidth for the reshuffles in PD-ORAM is 
$\order{log^{2}N}$ 
position map entries (Section \ref{oram:pdoram}). Considering $\order{logN}$ 
sized position map entries and $\Omega(log^{2}N)$ sized 
data blocks (a reasonable assumption by Stefanov {\em et al.} \cite{pathoram}), 
the total amortized bandwidth requirement for the reshuffle 
is equal to $\order{logN}$ data blocks. Since, in PD-ORAM the reshuffle for all 
levels is performed in the background without stopping
the queries, the 
additional bandwidth for each query due to to the reshuffle is thus bounded by 
$\order{logN}$.

In the case where the position map is stored recursively in RingORAMs, 
Stefanov {\em et al.} \cite{pathoram} show how to parameterize the recursion 
using non-uniform (smaller) blocks sizes for the position map ORAMs to 
achieve a bandwidth overhead of $\order{logN}$ to read a position map entry 
for a block. Therefore, using the PD-ORAM for storing position maps does not 
affect the overall bandwidth requirement for accessing data blocks from the RingORAM 
tree, which is critical to the performance of \sysname~.

\medskip
\noindent
{\bf Query complexity.~}
%
For a \sysname~ query, a client reads the stash, and a block from each of the $logN$ buckets 
on a particular path on the RingORAM tree. This has an overall access 
complexity of $\order{logN}$. Additionally, the client needs to 
read the data result log (DRL) which is $\order{e}$ in size . Note that the query log 
(which the client needs to read at the 
start of the query) is $\order{1}$ in size since it contains $e$ constant sized 
entries of a few bytes. Thus, with $e = \order{logN}$ the overall access  complexity for \sysname~ is 
$\order{logN}$. 


\medskip
\noindent
{\bf Eviction complexity.~}
%
For an eviction, the evicting client reads the append logs, the stash and all the buckets 
along a path on the tree.The append logs are bound by $\order{e} \in \order{logN}$ as shown 
before while the stash is $\order{logN}$ in size. The main overhead for the 
eviction is due to reading the buckets along the path where the bucket size, $z \in \order{logN}$. 
In this case, the complexity of reading the path is $\order{log^{2}N}$. Since 
the eviction is performed every $e = \order{logN}$ accesses, the amortized eviction 
complexity is $\order{logN}$.
\begin{small}
\begin{table*}
\centering
    \begin{tabular}{ | l | l | l | l | l | l | l |}
    
    \hline
    
    ORAM & Online (Query) Cost & Offline (Reshuffle) Cost & Client Communication Cost & Client Storage & Server Storage & Assumptions \\ 
\hline
      TaoStore~\cite{taostore}  & $\order{logN}$ & $\order{logN}$ & N/A & $\order{NlogN}$ & $\order{N}$ & Trusted Proxy\\
      Privatefs~\cite{privatefs} & $\order{logN}$ & $\order{log^{2}N}$ & N/A & $\order{\sqrt{N}logN}$ & $\order{NlogN}$ & N/A \\
      OPRAM~\cite{chenpram} & $\order{log^{2}N}$ & $\order{logN}$ & $\order{logc \times logN}$ & $\order{logN}$ & $\order{N}$ & Client Interaction	\\
      \sysname~	& $\order{logN + e}$ & $\order{logN + e}$ & N/A & $\order{\sqrt{N}logN}$ & $\order{NlogN}$ & N/a\\
      \hline
    \end{tabular}
    
    \caption{Asymptotic comparison of \sysname~ with other parallel ORAM constructions. Here, $e$ represents the eviction period for \sysname~ while $c$ represents 
    the number of parallel clients in the case of OPRAM~\cite{chenpram}.\label{asym_compare}}
\end{table*}
\end{small}

\medskip
\noindent
{\bf Asymptotic comparison with existing work.~}
%
Table~\ref{asym_compare} compares \sysname~ with existing parallel ORAM constructions. Note that OPRAM~\cite{chenpram} 
and PrivateFS~\cite{privatefs} have higher overall asymptotic overheads. TaoStore~\cite{taostore} requires 
higher client side storage to store the position map while {\em also operating under different assumptions and 
requiring the addition of a trusted proxy in-between.}

\medskip
\noindent
{\bf Security.~}
%
The security of \sysname~ is based on the security of the underlying RingORAM 
and PD-ORAM.
Each query in \sysname~ follows the same steps which are as follows:

\begin{enumerate}
 \item Append an encrypted entry to the query log and read the query log. The 
semantic 
 security of the encryption ensures that the server cannot learn the ID of the 
block 
 that is being queried.
 \item Read Stash. If the queried data block is found in the stash, then the 
client still proceeds with the following steps for indistinguishability.
 \item Read the corresponding position map entry from PD-ORAM. If the queried data 
block is found in the stash, then the client proceeds with a dummy 
access by reading  random buckets from each level. Security of PD-ORAM ensures 
that the server 
cannot learn the entry or the level in which the entry was found. Further, the 
uniformity of the hash function used to map entries to PD-ORAM buckets
ensures indistinguishability between buckets queried due to
a dummy access and a real access.
 \item Append the entry encrypted to the PM result log. For a dummy access, 
the client write back a fake entry. Semantic security of 
the  encryption used for PD-ORAM ensures indistinguishability of fake and real entries.
 \item Read a block from each bucket of RingORAM. If the client finds the 
queried block in the stash, then dummy blocks are read from all the buckets on 
the path.  
 The RingORAM access protocol \cite{ringoram} 
 ensures indistingishiability of dummy blocks from the real 
blocks and thus ensures that the server cannot learn the 
real block that was queried for by the client.
 \item Read the DRL after all previous clients finish (server 
enforced synchronization). 
 In the case 
where the client is waiting for another client to finish 
 accessing the queried block, reading the DRL after 
{\em all} previous queries have 
 completed ensures that  the server cannot learn which previous access the 
client was waiting for.
 \item Append a data block to the DRL after re-encryption. Semantic 
security of encryption ensures indistinguishability between the queried blocks 
and duplicates (if any).
\end{enumerate}

Evictions are performed by a single client with a lock on the data structures 
which prevents 
possible inconsistencies and leaks due to another client reading the path that 
is being evicted to. 
The DRL and the stash are merged locally and evicted to the 
deterministically (based on public information) 
selected path on the data tree. The eviction pattern, written data and locations 
are 
randomized and fully independent of client queries --
the server cannot learn the final distribution of blocks in the stash and tree. 


\begin{comment}
\begin{lemma}
 Accesses to the append logs are indistinguishable to an adversary and 
independent of the underlying queries.  
\end{lemma}

\begin{proof}
 Consider two concurrent queries $q_1$ and $q_2$ for data blocks, $b_1$ and 
$b_2$ respectively. 
 Both queries proceed by adding an encrypted entry to the query log serially. 
Consider $q_1$ starts execution 
 before $q_2$ and thus adds the corresponding entry to the query log before 
$q_2$. 
 This is followed by each query appending an encrypted position map 
 entry to the PM result log. If $b_1 = b_2$, $q_2$ appends a fake position map 
entry 
 indistinguishable from a real entry to the PM result log. 
  Then, the DRL is accessed after {\em all} previous queries finish. 
If $b_1 \neq b_2$ 
  $q_2$ reads the DRL after $q_1$ has finished, reencrypts and 
appends $b_2$. 
  If $b_1 = b_2$, $q_2$ finds $b_1$ in the DRL after $q_1$ has 
finished. 
  In this case $q_2$ reencrypts and 
  appends $b_1$. 
  Due to semantic security, the server only observes indistinguishable items 
being appended 
  to the logs independent of the outcome of the queries and the items being 
queried for.
\end{proof}
\end{comment}

% \smallskip
\begin{thm}
%
The existence of an adversary with a non-negligible advantage in violating
query privacy (as defined in \cite{goldreich}) for \sysname~ implies the
existence of an adversary with non-negligible advantage in violating query
privacy for PD-ORAM (``query privacy inheritance'').
%
\end{thm}

% \smallskip
\begin{proof}
% \proofsketch
% 
First, note that all \sysname~ queries look identical to the server and are
composed of the steps described above.

In effect, the server sees a transcript composed of a number 
of reads/writes on semantically secure encrypted data at fixed public and 
randomized locations (''randomized transcript") plus a PD-ORAM query.
 
Next, note that, if a client queries for a block that is being
simultaneously accessed by another client, it issues a fake query which is
indistinguishable from a real query.  Further, the server-enforced
synchronization, ensuring that clients waiting for simultaneous accesses to
finish accessing the queried block can obtain the most updated version of
the block from the DRL, is based on public knowledge -- the
order in which client connects (and appends entries to the query log).
 
Finally, consider an adversary $\mathcal{A}$ with non-negligible advantage
in violating query privacy for \sysname~.  An adversary $\mathcal{B}$
endowed with an equivalent advantage at violating query privacy for PD-ORAM
can be then constructed as follows: $\mathcal{B}$ simulates $\mathcal{A}$
for every query by appending random information to the append logs.  Since
the entries in the logs, the blocks read from the data tree and the
stash are encrypted with semantic security, any additional advantage to
$\mathcal{A}$ by observing these entries/blocks read from the path implies a
non-negligible advantage for $\mathcal{A}$ in distinguishing between the
output of the semantically secure encryption and random. Effectively, the
"randomized transcript" does not offer any non-negligible advantage.
$\mathcal{B}$ then outputs the guesses and requests provided by
$\mathcal{A}$, and obtains the same advantage as $\mathcal{A}$ (i.e., in the
query privacy game of \cite{goldreich}).

%
\end{proof}
 
 \begin{comment}
 Consider an adversary $\mathcal{A}$ with non-negligible advantage in violating 
query 
 privacy for \sysname~. We now construct an adversary $\mathcal{B}$ 
 endowed with an equivalent advantage at violating query privacy. $\mathcal{B}$ 
simulates $\mathcal{A}$ for every 
 query by appending random information to the append logs. Since the 
 entries in the logs are encrypted, any additional advantage to $\mathcal{A}$ by 
observing 
 the entries implies a non-negligible advantage for $\mathcal{A}$ in 
distinguishing between 
 the output of the semantically secure encryption and random. 
 Further, since $\mathcal{B}$ appends random information to the logs and all 
queries access PD-ORAM 
 and RingORAM (except for the logs, 
 any non-negligible advantage for $\mathcal{B}$ in violating query privacy 
implies a non-negligible advantage 
 for $\mathcal{B}$ in violating query privacy for RingORAM and PD-ORAM.
 \end{comment}

\begin{comment}
\begin{thm}
\sysname~ ensures MCCAS security and prevents correlation of concurrent queries 
and correlation of identical queries for data and position map entries before 
and after evictions.
\end{thm}

\begin{proofsketch}
 W.l.o.g consider a \sysname~ adversary, $\mathcal{A}$ selects $k=2$ in step 1 
of the MCCAS game and 
 sends $(x_1,y_1)$ and $(x_2,y_2)$ to \sysname~ clients $c_1$ and $c_2$. Further 
consider that on 
 the basis of a fair coin toss, $c_1$ and $c_2$ query for $x_1$ and $x_2$ 
respectively. 
 As discussed above, all queries follow the same steps in the \sysname~ 
 access protocol. Further, each step in the query protocol ensures that the 
server cannot 
 distinguish between queries for different items. Even in the case where $x_1 = 
x_2$ and $y_1 \neq y_2$, 
 $c_2$ retrives $x_1$ from the DRL (which would 
 be the case even for $x_1 \neq x_2$) only after $c_1$ has completed access, 
thus renderinging the two cases 
 indistinguishable. 
 
 Further, all access write the same number of encrypted items (either fake or 
real) to the append logs. 
 Semantic security of the encryption ensures indistinguishability of fake and 
real items. 
 Thus, the pattern of access for $x_1$ and $y_1$ are 
 indistinguishable to the server. Consequently, observing the access patterns to 
the RingORAM, PD-ORAM and 
 the logs, does not provide any advantage to the server in guessing whether 
$c_1$ has queried for $x_1$ 
 The same argument holds for any value of $k$ since query access pattern for a 
client is 
 independent of queries by other clients.
 
  For successive rounds of MCCAS, the eviction procedure ensures that accesses 
to the same 
 item $x_i$ never reads the item from the same location as the previous access. 
For a data block accessed 
 in the current round, the block is mapped to a randomly chosen new leaf in the 
RingORAM and is thus 
 subsequently read from a different path. For a position map entry, subsequent 
queries for the same position map 
 entry finds the entry either in the top level of PD-ORAM (which is always 
downloaded in its entirety 
 by the client for an access) or in a randomly chosen bucket in the other 
levels, as determined by a 
 uniform hash function. Thus, queries for the same item in rounds before and 
after an eviction result in independent 
 access patterns.

\end{proofsketch}
\end{comment}

 


==> figures/cloud_qr_gnuplot_ <==
set terminal postscript eps enhanced "Helvetica" 26 linewidth 1
set key left top
set output "cloud_qr.eps"
# set key top left font "Helvetica, 20"

# set terminal jpeg medium 
# set output "latency.jpeg"
set boxwidth 0.75 absolute
set style fill solid 1.00 border -1

set xlabel "Number of Clients"
set ylabel "Query Response Time(Milisecs)
plot "cloud_qr.dat" using 1:2 with lines title "ConcurORAM" linecolor rgb "red", \
     "cloud_qr.dat" using 1:3 with lines title "TaoStore" linecolor rgb "blue"


==> figures/plots/cloud_qr_gnuplot <==
set terminal postscript eps enhanced "Helvetica" 26 linewidth 1
set key left top
set output "cloud_qr.eps"
# set key top left font "Helvetica, 20"

# set terminal jpeg medium 
# set output "latency.jpeg"
set boxwidth 0.75 absolute
set style fill solid 1.00 border -1

set xlabel "Number of Clients"
set ylabel "Query Response Time(Milisecs)
plot "cloud_qr.dat" using 1:2 with lines title "ConcurORAM" linecolor rgb "red", \
     "cloud_qr.dat" using 1:3 with lines title "TaoStore" linecolor rgb "blue"


==> model.tex <==
\section{Background}
\label{model}

\subsection{Preliminaries}
%\smallskip


\noindent
{\bf Deployment.~} \sysname~ operates with two parties: the ORAM clients (with limited local storage) and the ORAM server (a remote storage hosting client data).

\begin{itemize}
	\item {\bf Honest-but-curious server}: The server does not deviate from the \sysname~ protocol. The server can observe  
	all requests and attempts to correlate them by saving and comparing snapshots.
	\item {\bf Trusted clients}: Clients are {\em honest} and share secrets (credentials, keys, hashes etc.) required for accessing the ORAM. Clients do not interact with each other.
		
%	As in numerous parallel multi-client ORAM constructions with a successfully established security model (PD-ORAM [21], PrivateFS, OPRAM [2,18]), \sysname~ considers {\em honest} clients that
%	do not interact with each other. Clients share 	
\end{itemize}

\medskip
\noindent
{\bf Notation.~} The server stores data as fixed-sized ``blocks''. \sysname~ considers $N$ 
blocks of outsourced data on the server. Blocks are 
addressed by logical block ID denoted by $id$. 
The logical address space for all blocks is shared by the clients.
The parties engage in an interactive query-response protocol established 
by \sysname~. The communication channel between the clients and the server is secured using TLS. 

%\smallskip
%\noindent
%{\bf Clients.~} As in numerous parallel multi-client ORAM constructions with a successfully established security model (PD-ORAM [21], PrivateFS, OPRAM [2,18]), \sysname~ considers {\em honest} clients that
%do not interact with each other. Clients share secrets (credentials, keys, hashes etc.) required for accessing the ORAM. 

%We note that separating {\em malicious} clients from each other requires stronger assumptions (such as trusted third-parties \cite{taostore}) and does not operate under the standard ORAM assumption of trust being only placed on clients at most.
%\sysname~ is not designed to separate clients from each other 
%and operates under the standard ORAM assumption of trust being only placed on clients at most.
%In contrast, TaoStore~\cite{taostore} considers an honest server but tolerates curious clients. Unfortunately, this introduces a large footprint assumption of a trusted close-to-server (proxy) executing queries on behalf of all clients to support inter-client isolation. This is rarely practical and does not really operate in a standard ORAM model, since significant trust is shifted away from clients.

%\smallskip
%\noindent
%{\bf Server.~} \sysname~ considers an {\em honest but curious} server that 
%does not deviate from the \sysname~ protocol. The server can observe  
%all requests and attempts to correlate them by saving and comparing snapshots (state of the 
%ORAMs after each query). The server implements and enforces the locks, counters etc. used in \sysname~\footnote{The server-side logic can be executed in a trusted execution environment~\cite{sgx} to ensure that the code is secure against tampering by other software running on the server.}.

%An ORAM controller implements 
%the \sysname~ server-side logic\footnote{\sysname~ assumes that the server  has basic computational capability for enforcing client synchronization, but this is not to be confused with complex homomorphic computations implementing the ORAM logic~\cite{onionoram}}. Specifically, the controller maintains (and duly increments) 
%access counters and arbitrates locks on shared data structures as required by the protocol
%\footnote{The ORAM controller can be executed in a trusted execution environment~\cite{sgx} 
%to ensure that the code is secure against tampering by other software running on the server.}. We use ORAM controller and server interchangeably  to refer to the same server-side component.
%\sysname~ does {\em not} consider a malicious server that can mount replay attacks and ``fork'' client views. Adapting the solution presented here to protect against a malicious server is ongoing work.
%

%\smallskip
\noindent
{\bf Network.~} 
%
Clients connect to the server through network links with similar 
bounded network delays. Our network model closely resembles the model used in \cite{privatefs}. 
Bounded network delay is a desirable feature for all ORAM constructions. This is 
because even asynchronous ORAM protocols (such as PD-ORAM~\cite{privatefs} and TaoStore~\cite{taostore}) 
need to ensure certain degree of synchrony to answer logical requests from clients in the order 
that they are received. \cite{privatefs} proves that enforcing this ordering 
of requests is necessary to ensure query privacy for ``non-simultaneous'' ORAMs 
that require serial execution of queries for the same underlying block.
In fact, \cite{taostore} describes an attack where violating this order allows 
the server to determine fake ORAM accesses from real ones based on the time when a 
query is answered. 

%Thus, with indefinite network delays, a client can be blocked for 
%significant periods of time before previous logical requests have been answered.

\begin{comment} 
{\bf Security challenge.~} Any system that supports multi-client concurrent access for ORAMs needs to prevent two possible security leaks -

\begin{itemize}
 \item Correlation between data items concurrently accessed in a single round.
 \item Correlation between data items accessed in successive rounds of one or more concurrent accesses.
\end{itemize}

Williams and Sion \cite{privatefs} prove that existence of an adversary 
with non-negligible advantage in violating query privacy for a ``parallel'' ORAM also 
implies the existance of an adversary with non-negligibility advantage in violating 
query privacy for the underlying ``single client'' ORAM. \sysname~ gaurantees multi-client 
concurrent access security by ensuring query privacy of concurrent accesses 
in each round using PD-ORAM and RingORAM as described in Section \ref{oram:overview}.



In the above context, we define multi-client concurrent access security (MCCAS) for ORAMs as a security game, where the challenger is 
a fixed set of clients, $\mathcal{C} = \{ c_1, c_2, \ldots c_n\}$, and the adversary, $\mathcal{A}$ is the remote server that hosts a database 
uploaded by $\mathcal{C}$. All items in the database are indexed and can be accessed concurrently by the clients. 

\begin{framed}
\begin{enumerate}
\item $\mathcal{A}$ and $\mathcal{C}$ engage in polynomial rounds of the following query-response based protocol
\begin{enumerate}
  \item $\mathcal{A}$ randomly selects $k \in [1,n]$. $\mathcal{A}$ selects $k$ pairs of item indices $(x_{i},y_{i})$,  such that 
  $i,j \in [1,k]$. $\mathcal{A}$ sends $(x_{i}, y_{i})$ to $c_{i}$.
  \item On the basis of a fair coin toss by $C$, bit $b$ is selected and sent to all $c_i, i \in [1,K]$. 
 \item If $b = 0$, client $c_{i}, i \in [1,k]$ queries for the item with index $x_{i}$. Otherwise, the client queries for the item with index $y_{i}$
 \item Observing the queries in Step 2, $\mathcal{A}$ outputs bit $b^{'}$
 \item $\mathcal{A}$ wins the round iff. $b^{'} = b$. 
 \end{enumerate}
 \item $\mathcal{A}$ wins the security game iff. she can win any round with non-negligible advantage over random guessing where non-negligibility is defined 
 over an implementation specific security parameter.
 \end{enumerate}
\end{framed}
 
A mechanism that satisfies the above security game ensures that it protects against the two aforementioned leaks. To see why consider the following: 

{\bf Correlation between data items accessed in a single round.~}
%
The security game straightforwardly ensures that $\mathcal{A}$ can win a round with non-negligible advantage over guessing if she can 
distinguish between two sequence of concurrent accesses. Therefore, a mechanism that satifies the game ensures that an adversary cannot correlate 
items concurrently accessed in the same round. 

{\bf Correlation between data items accessed in successive rounds.~}
Consider three randomly chosen pairs of item indices $(x_{1}, y_{1})$, $(x_{2}, y_{2})$ and $(x_{3}, y_{3})$. In two successive rounds, $\mathcal{A}$ provides the following 
pair to $c_{i}$:

\begin{itemize}
 \item Round1: $(x_{1}, y_{1})$ and $(x_{2}, y_{2})$
 \item Round2: $(x_{1}, y_{1})$ and $(x_{3}, y_{3})$
 \end{itemize}

In this case, if $c_{i}$ queries for $x_{1}$ (or $y_{1}$) both in round 1 and 2, and $\mathcal{A}$ could correlate accesses in the current round 
with previous rounds, $\mathcal{A}$ can win round 2 with non-negligible advantage. Therefore, a mechanism that satisfies the security game also ensures that 
an adversary cannot correlate accesses in successive rounds.

\end{comment}



==> parallelevictions.tex <==
\section{Parallel Background Evictions}
\label{oram:evictions}

Parallelizing the query step alone is not sufficient to achieve good
scalability.  Evictions are often very expensive and can block clients for
possibly impractical amounts of time.

%In fact, with larger buckets, evictions become even costlier than in
%PathORAM \cite{pathoram}, despite having the same asymptotic complexity. 
%For example, to perform $\order{logN}$ queries before an eviction, the
%bucket size also has to be $\order{logN}$, consequently leading to an
%$\order{log^{2}N}$ eviction complexity. Therefore, 
%even with parallel queries (Section \ref{oram:queries}),
%performing evictions while blocking queries limits the gains of parallelism.

To address this, \sysname~ introduces a new parallel eviction scheme with
two high level goals -- (i) multiple evictions can be performed in parallel,
and (ii) queries do not wait for ongoing evictions.  In particular,
evictions can be performed {\em asynchronously} ``in the background" without
blocking queries for significant periods of time\footnote{The two goals are
orthogonal and can also be achieved independently.}.

Without inter-client communication, maintaining consistency and correctness
across multiple parallel evictions is challenging.  This is because
evictions invariably update the same server-hosted data structures. 
Further, these data structures may be accessed not only by other evictions, but also by
ongoing queries.

A middle-ground efficient way to tackle this challenge, in the presence of
an honest-but-curious server, is to have multiple clients coordinate without
direct communication using server-hosted data structures.  As may be
evident, this role is performed by the append-only logs in
Section~\ref{oram:queries}.  Now we extend the idea for parallel evictions.

To this end, we first analyze and identify portions of the eviction protocol
(Section~\ref{oram:queries}) where synchronization is absolutely critical. 
These steps can then be performed with fine-grained locking while steps that
do not require direct inter-client locking are performed in parallel using
server-hosted data structures designed to maintain state and enforce
minimally-sufficient global serialization.
%
%.
%For example, with evictions performed in parallel to multiple paths in the
%data tree, buckets that are part of more than one such eviction path will be
%updated concurrently by clients performing the evictions. This 
%will lead to inconsistencies unless handled carefully.  Also, since the
%outcome of an eviction depends on the state of the system after previous
%evictions have completed, a smart global notion of synchronization has to be
%enforceable inherently.

We start by describing how to perform {\em one} eviction in the background
without blocking ongoing queries.  In Section \ref{oram:evictions_parallel},
the idea is extended to multiple asynchronous evictions.

\subsection{Non-blocking evictions}
\label{oram:evict_background}

In the non-parallel case (Section \ref{oram:queries})
evictions include the following ordered steps client-side: (i) fetching
buckets from a path of the data tree (eviction path), (ii) evicting contents
of the stash and creating a new path locally, (iii) writing back the new
path to the tree and uploading the new stash, and (iv) updating the position
map (PD-ORAM) and clearing logs.

Further, the query protocol (Figure~\ref{query_overview}) includes the
following client-side steps: (i) updating query log, (ii) reading the stash
and position map query (PD-ORAM), (iii) fetching the query path from the
data tree, and (iv) reading and updating the data result log.

Now, note that eviction steps (i) and (ii) collectively read a specific path
from the data tree and the stash, and perform local computation.  These
steps do not update the server-hosted data structures and are not in
conflict with query protocol steps.

Eviction step (iii) however updates the data tree and the stash -- read in
Steps (ii) and (iii) of the query protocol -- and requires mitigation and
possible synchronization.  {\em One idea here is to perform queries on a
read-only copy of these data structures while the updates performed to the
data tree and the stash during the evictions happen on a writable copy never
accessed by the queries}.  Once the eviction completes updating the writable
version of the data tree and stash, the contents can be copied to the
read-only data tree and stash, and made available for future queries.

%\smallskip
\noindent
{\bf Write-Only Tree.~}
%
Specifically, a write-only tree (``W/O tree'') is initialized with the same
contents as the read-only data tree.  The W/O tree is updated during
evictions while the data tree is used to satisfy queries in the background. 
This is possible because queries do not update the data tree and queried
blocks that are updated with new data make it back to the data tree only
during evictions.
%
% (inherently read-only)
%\todo{queries do not involve updates? in ORAM usually query means anything}



%\smallskip
\noindent
{\bf Temporary Stash.~}
% 
Further, during the eviction of blocks along a specific path of the W/O tree
(eviction path), blocks that cannot be accommodated are placed in a
``temporary stash'' (not accessible to queries) on the server.
% 

Then, once the entire eviction path is updated, the path is copied from the
W/O tree to the data tree, and the temporary stash is made available for
queries by replacing the main stash with the temporary stash.  Note that at
this stage the contents of the main stash have already been evicted to the
data tree and the temporary stash, and thus can be replaced without any data
loss.


%\todo{is it replacing the main stash? what does made available mean?
%please think of a 5 year old nephew.}

%Once the W/O tree has been updated,  \todo{which path?! explain} 
%\todo{what is a stash of a tree and is this shared between clients? why are
%we bringing it up here? does it require synchronization?} 

While the eviction path is being copied from the W/O tree to the data tree, {\em new} queries -- queries that are waiting to register an
entry in the query log (Step 1 of the query protocol,
Figure~\ref{query_overview}) -- need to be blocked to avoid possible
conflicts.  This is enforced using the query lock (Section \ref{oram:queries}), needed for updating both the data tree and the stash.

%Finally, after copying the path, updating PD-ORAM (creating the top level
%from items in the data result log), and updating the main stash (replacing
%it with the temporary stash), an eviction {\em commits} by clearing all logs.

More formally, and importantly, \sysname~ splits evictions into two {\em
phases that can be performed in parallel by different clients} --

\noindent
{\bf Processing.~}
% \todo{explicited each action separately} 
%
% The processing phase performs the following -- 

\begin{enumerate}
	\item Fetch buckets from the eviction path on data tree 
        \item Fetch current stash
	\item Evict contents of the stash + eviction path
        \item Create a new path and temporary stash locally 
	\item Write back the updated path to the W/O tree
        \item Write back the temporary stash to the server
\end{enumerate}

%Figure~\ref{xxxx} 

\noindent
{\bf Commit.~}
%
% The commit phase performs the following -- 

\begin{enumerate}
	\item Update the position map PD-ORAM (create the new top level with position map entries for the blocks that have been evicted to the W/O tree). 
	\item Copy the eviction path from the W/O tree to the data tree.
	\item Replace the contents of the existing main stash (which was previously used to satisfy queries) with the contents of the temporary stash. 
	\item Clear the query log 
        \item Clear the data result log
\end{enumerate}


%Figure~\ref{xxxx}


\begin{figure}
	\includegraphics[scale=0.11]{figures/transaction_schedule.eps}
	\vspace{-7.5cm}
\footnotesize{\caption{(a) For non-parallel ORAMs, queries are followed by an
expensive eviction step. (b) In \sysname~ evictions are divided into a
processing phase and a significantly less expensive commit phase.  Queries
can be executed in parallel with the processing and wait only a short time
for the commit.} \label{transact_sched}}
\end{figure}




%\smallskip
\noindent
{\bf Locking mechanism for commits.~}
%
Fine-grained locking is necessary to maintain consistency.  Eviction commits
first acquire the query lock and thus block new incoming queries from proceeding
(new queries need to acquire the same lock in Step 1 of the query protocol). 

Further, all {\em ongoing queries} -- queries that have registered an entry
in the query log, but have yet to finish all the steps of the query protocol
-- need to finish before an eviction can update shared data structures (data
tree, stash etc.).  In other words, \sysname~ does not ``preempt'' ongoing
queries to perform eviction commits.

To ensure this, after an eviction acquires the query lock, it waits for the
ongoing queries to finish.  Because {\em all} queries start execution by
registering an entry in the query log (Step 1 of the query protocol), and
finish by adding a block to the DRL (Step 7) -- the number of ongoing
queries yet to finish can be determined by comparing the sizes of the query
log and the current DRL.

\noindent
{\bf Degree of parallelism}
%
As may be evident, commits only involve local copies between server-side
data structures.  Because of this, {\em commits are not impacted by network
bandwidth}.  On the other hand, the processing phase updates an entire path
of the W/O tree, incurring a bandwidth overhead of $\order{log^{2}N}$.  

To significantly increase parallelism, \sysname~ maintains a judiciously
optimized transaction schedule (Figure \ref{transact_sched}) interleaving
commits and processing.

{\em New} queries end up waiting to acquire the {\em query lock} during the
commit phase.  In turn, an eviction may be waiting for a round of queries to
finish before being able to commit.

So, in the worst case, a new query may have to wait for a round of {\em
parallel} queries to finish in addition to an eviction commit (executed by another client).  Since the steps of the query protocol are performed in parallel, the time required to complete a round of $c$
(determined by the log size) parallel queries is not significantly higher
than the time required to complete a single query (Section
\ref{oram:queries}). Also, eviction commits are inexpensive as discussed above.
%
%Also, a query waits for the eviction commit executed by another
%client (but not the eviction processing).

The significantly more expensive (by a factor
of $\order{logN}$) processing phase can be executed in the background
without blocking queries or commits.

%%\todo{``wait for a round of queries'' sounds very long -- what is a
%%round of queries? all of the queries to complete? it seems anti-parallelism} 
% \todo{``i.e., 
%'?} . 
%%\todo{this is super confusing!!! the lock is a
%%mutex lock or is something else like a semaphore? In either case I am unsure what else the server does here.
%%The server should not have to do anything explicitly -- the eviction code
%%simply acquires and releases locks no?!?! -- this is very very
%%confusing.}
%
%\smallskip
\noindent
{\bf Storing and privately accessing query results.~}
%
Blocks that have been previously accessed but not yet evicted to the data
tree need to be stored somewhere.  Since background evictions may require
longer periods of time, results generated by queries must be stored until
the next eviction.  

In particular, each round of parallel queries that is executed in the
background while an eviction takes place, will generate a DRL containing the
blocks that have been accessed by the queries.  Until the contents of the
DRLs can be evicted back to the data tree (which can then be accessed by
queries in the future), the DRLs need to be maintained separately on the
server.  Also, since reading all such DRLs in their entirety in Step 6 of
the query protocol (Figure \ref{query_overview}) would certainly be
expensive, we need to devise a mechanism to efficiently query for particular
items from the DRLs without leaking their identity to the server.  This is
achieved by the {\em DR-LogSet} structure.

%This can be handled by filling new server-side
%\todo{does it make sense to call them temporary logs?} logs with
%results of the ongoing queries, while data is evicted from the DRL\todo{very
%confusing -- are these ``logs'' the DRLs or something else? you need to
%gently and clearly explain this step by step}.  The
%challenge then is to maintain these logs efficiently while also ensuring a
%way to securely query the items within them. 

%This requires an ability to maintain and access all these individual logs for satisfying future queries.  
%%generates a ``log of logs''. \todo{is this described somewhere? 
%%are these logs individual per client? where is this log of logs -- or is this an abstract construct ? in that case
%%you cannot say ``this generates'' and instead we need to say something like
%%-- ``this requires an ability to handle all these individual logs'' or
%%something to that effect}
%%However, it is impractical to access \todo{why is it impractical?!} the entire
%%``log of logs'' for queries. 

% 
% even though I understood some of this later, I left all questions in as
% they came to my mind since reviewer will also have the same questions

%\smallskip
\noindent
%
{\bf DR-LogSet.~}
%
The DR-LogSet includes the current DRL (of size $c$), and $k \leq c$ DRLs
generated by rounds of queries that finished execution while an eviction was
being performed in the background.  Except for the current DRL, all other
previously generated DRLs are stored in the DR-LogSet as ``bigentry logs'' of
size $2c$ -- each bigentry log is composed of a random permutation of the
(re-encrypted) blocks of a previously generated DRL combined with an
additional $c$ (or more) random dummy blocks.

``Bigentry logs'' are ordered by ascending insertion time, $l_{1}, l_{2},
\ldots, l_{k}$, with $l_{k}$ being the ID of the log inserted most recently.
A search index is appended to track the location of data and dummy blocks in the
randomly permuted log. 

The idea here is to read the current DRL in its entirety in Step 6 of the
query protocol, as well as obliviously access {\em one unique} block each
from the bigentry logs (as determined by their search index).

More specifically, if the block required by the query is in one of the
bigentry logs, it is read from there, otherwise a {\em unique} dummy block
is read.  Due to the random permutation of (encrypted) dummy and real
blocks, the two cases are indistinguishable.

Further, each bigentry log is reshuffled randomly (and its dummy blocks
refreshed) at least once in $c$ accesss, thus ensuring it does not run out
of {\em unique} dummy blocks. 




\begin{small}
	\begin{algorithm}
		\caption{writeLogSet($blk$)}\label{writelogset}
		\begin{algorithmic}[1]
			\State $blk$:  Queried block to be appended to DRL
			\State $i$: Current size of DRL
			\If {$i < c - 1$}
				\State Append encrypted $blk$ to current DRL
				\item[] \begin{center} (Steps performed in Background) \end{center}
				\State $l_{i+1}$: Get $(i+1)^{th}$ bigentry log from DR-LogSet
				\State $l_{i+1}$.reshuffle(rand)
				\State Write back $l_{i+1}$ to the {\em Reshuffled-LogStore}
			\Else
				\State $l_{i+1}$: Get $(i+1)^{th}$ bigentry log from DR-LogSet 
				\State $l_{i+1}$.reshuffle(rand)
				\State Write back $l_{i+1}$ to {\em Reshuffled-LogStore}
				\State // Replace {\em all} bigentry logs in the DR-LogSet with their reshuffled versions in the {\em Reshuffled-LogStore}
				\If{less than $c$ bigentry logs in DR-LogSet}
					\item[] \begin{center} (Create new bigentry log) \end{center}
					\State $j$: Number of logs in the DR-LogSet 
					\State Initialize $l_{j+1}$ with size $2c$ blocks
					\State $l_{j+1} = blk + drl_{curr} + dummy$
					\State $l_{j+1}.reshuffle(rand)$
					\State // Append search index to $l_{j+1}$
					\State // Reencrypt and write back $l_{j+1}$ to the DR-LogSet
					\State // Initialize empty DRL for new round of queries
				\Else
					\item[] \begin{center}(Wait until next eviction commit)\end{center}
				\EndIf	
			\EndIf 
		\end{algorithmic}
	\end{algorithm}
\end{small}


This is performed as part of $\mathbf{writeLogSet(blk)}$ (Algorithm \ref{writelogset}) which is also used by a client to append the queried block the current DRL in Step 6 of the query protocol. The algorithm first checks the current size of the DRL. If the number of blocks currently in the DRL is $i < c-1$ (Step 3), the queried block ($blk$) is appended to the DRL. 

 Then, the client reshuffles $(i+1)^{th}$ bigentry log from the DR-LogSet {\em in background} (Steps 5 - 7). More specifically, the bigentry log is read from the DR-LogSet, the blocks are reencrypted and reshuffled randomly (Steps 5, 6). Note that in some cases the DR-LogSet may contain less then $i+1$ bigentry logs, in which case a reshuffle will not be performed. The reshuffled bigentry log is written to a temporary location on the server, allocated specifically for storing the reshuffled bigentry logs until they can be added back to the DR-LogSet. This is called the {\em Reshuffled-LogStore}. The contents of the Reshuffled-LogStore are not available for queries.
 
 The Reshuffled-LogStore enables performing the bigentry log reshuffles in the background without interfering with the ongoing queries. This is important since after the queried block is appended to the DRL in Step 4, the queries waiting for access to the DRL (Step 5 of the query protocol) can proceed without waiting for the bigentry log reshuffle to finish. 
 
 
The reshuffled versions of the bigentry logs (in the Reshuffled-LogStore) replace the old versions in the DR-LogSet once the current DRL is full (Step 9 - 12). Since the size of the DRL is $c$ and there can be a maximum of $c$ bigentry logs in the DR-LogSet, this ensures that each bigentry log is reshuffled at least once within $c$ accesses
The Reshuffled-LogStore is subsequently cleared.

Additionally, when the current DRL is full (Step 8), the client initializes a new ``bigentry log'' with $2c$ blocks (Step 14-15).  The block queried by the client and the up-to-date blocks from the current DRL are added to the newly created bigentry log while filling up the remaining part with dummy blocks (Step 16).  The encrypted bigentry log entries are shuffled randomly and a search index is appended to track locations of real data blocks and dummy blocks.   This bigentry log is finally added to the DR-LogSet (Step 17-20) and a new DRL is initialized for the next round of parallel queries. 

Data blocks of the DR-LogSet bigentry logs are eventually evicted to the data
tree by future evictions.  Specifically, once the current eviction
completes, the next eviction will evict blocks from the ``oldest'' bigentry log. Therefore, 
if the DR-LogSet already contains $c$ bigentry logs, a new log cannot be added until at least one eviction completes (Step 20).

%
%$\mathbf{writeLogSet(blk)}$ appends block $blk$ to the current DRL. 
%Further, if $blk$ is the $i^{th}$ block in the current DRL ($i \leq c$) the
%client also reads and randomly reshuffles ``bigentry log'' $l_{i}$ from the
%DR-LogSet (Steps 3 - 5 in Algorithm \ref{writelogset}).  This
%ensures that by the time $c$ blocks have been appended to the current DRL
%(and the DRL is full), {\em all ``bigentry logs'' in the DR-LogSet have been
%reshuffled at least once}.
%
%If the current DRL fills up after appending $blk$, 


% \todo{``oldest''?} 
%% that was added before all the other bigentry logs. 
%\todo{why oldest? maybe youngest?}


\begin{small}
	\begin{algorithm}
		\caption{readLogSet($id$)}\label{readlogset}
		\begin{algorithmic}[1]
			\State $DRL$: Read current DRL
			\For{$i \in [k, k-1, \ldots, 1]$}
			\State $index\_blk$: Read search index for $l_i$
			\If {$id \in index\_blk$}
			\If{$id \notin DRL$}
			\State Read block $id$ from $l_{i}$
			\State Remove $id$ from $index\_blk$
			\Else
			\State Read $dummy$ from $l_{i}$ 
			\State Remove $id$ and $dummy$ from $index\_blk$
			\EndIf
			\Else
			\State Read $dummy$ from $l_{i}$
			\State Remove $dummy$ from $index\_blk$
			\EndIf 
			\State Reencrypt and write back $index\_blk$
			\EndFor
		\end{algorithmic}
	\end{algorithm}
\end{small}

% 
For reading blocks from the DR-LogSet in Step 7 of the query
protocol, $\mathbf{readLogSet(id)}$ (Algorithm \ref{readlogset}) reads the
current DRL and {\em one} block each 
from the bigentry logs in {\em descending order} of log ID -- recent
logs are read before old ones.  If the queried block ID $id$ is present in a
bigentry log as determined from the corresponding search index (Step 4)
and the block is not present in the current DRL, it is retrieved from the
bigentry log and ID $id$ is removed from its search index (Steps 5 - 7). 
On the other hand, if the block is also present in the current DRL, a dummy
block is read from the bigentry log and $id$ is removed from the search
index along with the entry for the dummy block (Steps 8 - 10).  Finally, if
the queried block is not in the bigentry log, a dummy
block is read and the corresponding entry is removed from the search index
(Steps 11 - 13).  Note that the entries from the search indices are removed
client side, and the updated index is placed back on the server after being
reencrypted with semantic security -- the server cannot identify entries
that have been removed.

%\todo{removing stuff from
%indexes etc is done client side and stuff gets placed back encrypted on the
%server so the server doesn't know?  maybe this needs 1 sentence at least
%here}
%
Further, note that due to the round robin reshuffling of the bigentry
logs as part of $writeLogSet$, a bigentry log is accessed at most $c$ times
before it is replaced by an independently reshuffled version of the log (from the Reshuffled-logStore).  This limit is important -- as each log
contains at least $c$ dummy blocks, a different dummy block can be read for
each of the $c$ accesses before the next reshuffle.   
Since entries
corresponding to blocks (including dummy blocks) that have been read once
are removed from the search indices, unique blocks are read from the logs
for each of the $c$ accesses. 

Due to the request order based synchronization (Step 5 of the query protocol), clients access the DR-LogSet serially -- client queries wait for all previous queries to finish  reading (using $readLogSet(id)$ in Step 6) and updating (using $writeLogSet(blk)$ in Step 7) the DRL before it proceeds with its own access.
Therefore, consistency of the DR-LogSet is ensured while 
 modifying indices (during reads) and replacing the bigentry logs (during the writes),  without explicit locking.
 


\begin{customlemma}{1}
\label{drl_lemma}
%
The accesses to the DR-LogSet produce transcripts that are indistinguishable
and independent of the block that is being queried.
% 
\end{customlemma}

Proof in Appendix.
 
\subsection{Parallel Evictions}
\label{oram:evictions_parallel}

Since evictions can require long periods of time, several rounds of queries
can be performed in parallel, each adding a bigentry log to the DR-LogSet.  If blocks
are evicted to the data tree from only a single bigentry log at a time, the
DR-LogSet will become unbounded soon because by the time a bigentry log is cleared from the DR-LogSet, several new bigentry logs will have been created. To ensure that the DR-LogSet remains bounded to an acceptable size, evictions must start as soon as a
``bigentry'' log has been added, even if a previous eviction has not
finished.  In this case, multiple evictions will need to be executed in
parallel.

%
%Consequently, multiple evictions 
%will execute in parallel\todo{this is not in a ``consequent'' relationship
%with the previous phrase. It is at most related. Why say ``cponsequently''?!?!?!
%Or do you mean ``need to execute in parallel''? Even then it is not
%consequent but it makes a bit more sense}.

Facilitating parallel evictions is challenging due to overlapping accesses
to the W/O tree.  More specifically, two independent paths being evicted to
in parallel will invariably intersect at some level of the W/O tree. 
Updates to any buckets residing on the intersection of the paths need to be
synchronized.


\begin{figure}
	\centering
	\includegraphics[scale=0.12]{figures/EST.eps}
	\vspace{-0.5cm}
	\footnotesize{\caption{Eviction subtree (EST) defined by 4 parallel eviction clients evicting to paths in the reverse lexicographical order of their leaf IDs.\label{est}}}
\end{figure}

\noindent
{\bf Reverse lexicographical ordering of eviction paths.~}
%
Recall from Section~\ref{oram:queries} that evictions are performed to paths
in the data tree in reverse lexicographical order of their corresponding
paths' leaf IDs, similar to RingORAM~\cite{ringoram}.

Before we proceed further, it is important to understand how this works. 
The reverse lexicographical representation used in \sysname~ (and in
\cite{ringoram}) denotes each path of the data tree as a {\em unique} binary
string.  The least significant bit (LSB) of the string assigned for a path
is 0 if the target leaf corresponding to the path is in the left subtree of
the root and 1 otherwise.  The process is continued recursively for the next
bits, up until reaching the leaf, with the next bit(s) being assigned based
on whether the leaf is in the left or right subtree of the children nodes
\cite{ringoram}.

\sysname~ uses a counter to track the number of evictions that have taken
place since initialization.  If the current value of the counter is, say
$ctr$, the next eviction will be to the path that has a reverse
lexicographical representation matching the binary representation of $(ctr +
1)\bmod N$. Intuitively this results in all $N$ paths of the tree being selected once before the same path is selected again for eviction.  In general, $k$ successive evictions are to paths that have
reverse lexicographical representations matching the binary representations
of $(ctr+1) \bmod N, \ldots (ctr+k) \bmod N $ respectively.

Since each path is represented by a {\em unique} lexicographical
representation, any $k$ successive eviction paths are deterministic.  Further, if
only these $k$ evictions are allowed to execute in parallel, then the
overlaps between the paths can be predicted precisely.  As we
show next, if the maximum number of evictions that can be executed in
parallel is fixed at initialization, to say $k$, we can define a maximal subtree outside of which the $k$ successive eviction paths will never overlap in the W/O tree.
 
Now, to continue we need to first present a related result.

\begin{customthm}{2}
\label{thm:rev_lex}
% 
 The length of the longest common suffix between the binary representations of any
 $k \leq N/2$ consecutive integers selected from the integer modulo group of
 $N$, i.e.  $\{0,1, \ldots, N-1\}$, is bounded by $\log{k}$.

\end{customthm}

Proof in Appendix.
%\todo{pls. clarify proof}

Note that the actual values of the $k$ integers do not matter as long as
they are consecutive in mod $N$.

\noindent
% 
{\bf Eviction subtree (EST).~} 
%
Note that to select the next eviction path, \sysname~ calculates $v = (ctr +
1) \bmod N$ -- thus any $k$ consecutive values of $v$ (i.e., corresponding to $k$
sequential evictions) are consecutive integers in $\bmod N$.

Then, theorem \ref{thm:rev_lex} provides a critical insight: given any two
values within the next $k$ consecutive values of $v$, say $v_1$ and $v_2$,
the binary representations of $v_1$ and
$v_2$ cannot have a common suffix of length greater than $\log{k}$.

And, as the values of $v$ are used to determine any $k$ successive eviction paths by
matching them with the reverse lexicographical representations of data tree
paths (as described before), the length of the longest common suffix between
the reverse lexicographical representations corresponding to any $k$ successive eviction paths cannot exceed $\log{k}$. 

Due to the way in which the lexicographical representation of a path is
assigned (described above), the length of the common suffix between the
reverse lexicographical representation of two paths has a certain
significance -- it corresponds to the levels of the tree (from root to leaf)
where the paths overlap.  So $k$ parallel evictions that started in
succession, can overlap with each other on at most the first $\log{k}$ levels of the
tree. 
%
%If the maximum number of parallel ongoing evictions is bounded to an integer $k$, then the reverse lexicographical representations of paths to which the $k$ (consecutive) evictions take place have a longest common suffix that does not exceed a length of $logk$. Further, due the way in which the lexicographical representation of a path is assigned (described above), the common suffix between the reverse lexicographical representation of two paths has an important physical significance -- it corresponds to the levels of the tree (from root to leaf) where the paths overlap. So $k$ parallel evictions that started in succession, can overlap with each other only up to $logk$ levels of the tree, irrespective of the paths they are evicting to (Theorem \ref{thm:rev_lex}).

\sysname~ fixes the maximum number of parallel evictions that can be
executed at a time, $k \leq N/2$, during initialization.  In general, this should be
set to the number of parallel clients.

Further, consider that out of all the evictions being executed in parallel,
the eviction that began execution before all the others, say $e_i$, started
when the eviction counter was at $c$.  Then, \sysname~ enforces that the
eviction counter does not exceed $c+2k$ before $e_i$ completes.

More formally, let $ctr_{1}, ctr_{2}, \ldots ctr_{k}$ be the respective
values of the eviction counter when the $k$ parallel executions started
execution.  \sysname~ enforces that for any $ctr_i$ and $ctr_j$, where $i,j
\in (1,2,..,k)$, $ctr_{j} - ctr_{i} \leq 2k$.  Theorem \ref{thm:rev_lex} can
be straightforwardly extended to show that for $2k$ consecutive integers in
the modulo group of $N$, the length of the longest common suffix between
their binary representations will be bounded by $\log{k+1}$.  So following the
discussion above, it should be clear that the at any given time, the next
$2k$ parallel eviction paths based on the eviction counter values can only
intersect on at most the first $\log{k+1}$ levels of the data tree.

%\todo{``at most'' or ``exactly''?}

%By the extension of  Theorem \ref{thm:rev_lex}, the length of the longest common suffix between the binary representations of any such pair of counter values is bounded by $logk+1$. Since the reverse lexicographical representations of the eviction paths matches the binary representation of the counter values, this implies that .

Accordingly we define the eviction subtree (EST) as the subtree
of the W/O tree containing the root and the buckets overlapping between the
parallel eviction paths.  For $c$ parallel eviction, the height of the EST
is $h  = \log{c+1}$. Figure \ref{est} shows an example EST with 4 parallel evictions. 

%\begin{center}
%	$h  = \log{c+1}$
%\end{center}




%To facilitate this, \sysname~ 
%
%
%
%We can combine this information with the knowl
%edge of the number of parallel
%ongoing evictions, to {\em exactly} determine the overlapping buckets on the
%intersecting paths.  In particular, each successive eviction is executed on a deterministically chosen path. 
%So, if $k$ evictions that started successively one after the other are executing in parallel, given the number of evictions that have already taken place, we can precisely determine the $k$ eviction paths. This gives the intersecting buckets.
%
%Further, selecting eviction paths based 
%on the reverse lexicographical ordering of leaf IDs ensures minimum overlaps between successive 
%evictions \cite{ringoram}. More specifically, if $e_i$ evicts 
%to a path in the  left subtree of the root in the data tree, $e_{i+1}$ necessarily evicts to a path in the right subtree. More importantly, this holds for any $ 2 \leq k < N$ successive evictions. 
%
%\todo{completely unclear?  why can we do this?  some
%intuition.  think literally of a 5 year old nephew!  please write for a 5
%year old!}

While writing back to the W/O tree, evictions access the buckets in the EST
only after acquiring the {\em processing lock}.  Specifically, updating the
EST and uploading the temporary stash is the critical section and is
performed atomically by only one eviction at a time.  The rest of the path
can be updated asynchronously.

%Also note that the order in which evictions enter the critical section is
%then implicitly used later to serialize commits (discussed later).

%However, in general evictions are designed to be synchronous. This is because the outcome 
%of an eviction defines the state of the ORAM for future queries. Multiple evictions 
%executing in parallel without synchronization will lead to inconsistent states of the shared dataread-only set. 

% structures.
%
%%\smallskip
%\noindent
%{\bf Serialized processing.~} 
%%
%Accesses to shared data structures  (e.g., stash, intersecting buckets on path etc.) can be synchronized by enforcing a logical serial 
%order on concurrently-executing eviction clients, while performing
%steps that access them.  Moreover, once
%this serial order has been established, to ensure a consistent system state, evictions should ideally also commit serially, since the
%outcome of an eviction depends on the outcome of the previous evictions.
%


%\smallskip
\noindent
{\bf Server-side cache.~}
%
Note that contents written by a particular eviction to the actual EST may be
overwritten by subsequent overlapping evictions before the
particular eviction finally commits.  The {\em server-side cache} persists these
contents.  Once the eviction commits, the contents in the corresponding
server-side cache are invalidated and it can be allocated
elsewhere.

\sysname~ provides per-eviction server-side caches active
until the evictions commits.  Specifically, each eviction is assigned its
own server-side cache with two components --

\begin{enumerate}
	\item EST buckets written back along the eviction path to the W/O tree.
	\item The temporary stash created during eviction.
\end{enumerate} 




\noindent
{\bf Processing.~}
%
Processing incorporates several changes to support parallel evictions. It is 
divided into the following three stages (Figure~\ref{evict_process}) -- 

\begin{enumerate}

\item Stage 1 -- Read the non-EST buckets on the eviction path from
the W/O tree.

\item Stage 2 -- A critical section which requires acquiring the
processing lock, $L_{p}$ -- only one eviction can be in the critical section
at a given time.  It includes the following sub-steps:

	\begin{enumerate}

	\item Read the temporary stash uploaded by the eviction that {\em
	last} executed the critical section.  This is separately maintained on the
	server (``most recent temporary stash'' in Figure~\ref{evict_process}).

	\item Read buckets in the EST along the eviction path from the W/O Tree.

	\item Write back updated buckets to the EST along the eviction path, and the temporary stash

	\end{enumerate}

\item Stage 3 -- Write back non-EST buckets on the eviction path to the W/O tree.
	
\end{enumerate}

Note that the processing lock acquired in Stage 2 only protects the EST
buckets in the W/O tree, since locking the entire tree is not necessary for
consistency (as discussed before) and would block evictions in Stage 1 and
Stage 3.

Further, note that an eviction executing in Stage 1 does not overlap with
any eviction in Stage 3 since all ongoing parallel evictions can overlap
only in the EST.

\begin{figure}
	\centering
	\includegraphics[scale=0.045]{figures/eviction_process.eps}
\vspace{-0.3cm}
	\footnotesize{\caption{Eviction processing is divided into the three
	stages.  Stage 1 and 3 read and write back the eviction path
	respectively.  An eviction executing in Stage 1 does not overlap
	with any eviction in Stage 3 since all ongoing parallel
	evictions can overlap only in the EST (as the maximum number of
	ongoing evictions is fixed at initialization).  Stage 2 is the
	critical section and is accessed after acquiring the processing
	lock.  The execution of the critical section defines an ordering of
	evictions, which is used later to serialize
	commits.\label{evict_process}}}

\end{figure}



%\smallskip 
%\smallskip
\noindent
{\bf Serialized commits.~}
%
Updates performed in the critical section determine the state of the system
for future evictions and queries.  This is because an eviction that enters
the critical section, uses results (EST buckets, temporary stash etc.)
generated by the previous eviction that entered the critical section.  Thus,
{\em if commits are serialized based on the order in which evictions execute in
the critical section, additional synchronization is not necessary} to ensure
consistency of data structures updated during the commit.  Unfortunately,
serialized commits may result in unnecessary and prolonged waits.

To provide the full benefits of parallelism, \sysname~ allow asynchronous
eviction commits -- concurrent evictions can commit in any order, but
information from each eviction is persisted in multiple shared data
structures, and judiciously reconciled later (cleared when other preceding
clients in the serial order also finish their commits).

%\smallskip
\noindent
{\bf StashSet.~}
%
With serialized commits (Section~\ref{oram:evict_background}), the temporary
stash created by an eviction can straightforwardly replace the main stash
and satisfy future queries after the commit.  

However, unfortunately, this is not the case when evictions commit asynchronously. 
For example, consider an ordering of evictions established by the execution
of the critical section -- $e_{i-1} < e_{i} < e_{i+1}$.  Also, let $e_{i+1}$
commit when $e_{i-1}$ has committed but $e_{i}$ is yet to commit.  In this
case, contents that are evicted to a path, $p_{i}$ by $e_{i}$ from the
temporary stash created by $e_{i-1}$ (denoted by $TempStash_{i-1}$), will
not be available for queries until $p_{i}$ is updated in the data tree. 
Thus, replacing $TempStash_{i-1}$ with $TempStash_{i+1}$ as the main stash
will lead to data loss.

To overcome this, instead of storing a single stash, \sysname~ stores a set
of temporary stashes created and uploaded by evictions that have committed
asynchronously before previous evictions could be completed.  Each temporary
stash is assigned a unique ID as described below.
% \todo{``and will be judiciously
%reconciled later with all other temporary stashes''?}.

The curious but non-malicious server stores a counter tracking the
number of evictions that have executed the critical section since
initialization, the {\em processing counter}.  While in the critical
section, an eviction reads the value of the processing counter, which
becomes its {\em temporary eviction ID}.  Before exiting the critical
section, the processing counter is incremented.  \sysname~ assigns temporary
stash IDs based on the {\em temporary eviction ID} of the eviction that
created it.  In other words, if an eviction has {\em temporary eviction ID}
$i$, the temporary stash created by the eviction is denoted as $TempStash_i$
and its unique Stash ID is $i$.

%The StashSet stores stashes in order of $TempStash_{i}, TempStash_{i+1}, \ldots, TempStash_{i+k}$ ($TempStash_{i+k}$ being the most recently added).
%On a commit, the temporary stash created by the eviction is added to the StashSet. In case, the 
%all previous evictions (order established by access to critical section) have committed, the 
%temporary stash becomes the current stash. As a consequence, client queries must query the entire
%StashSet efficiently instead of only the current stash. We first formally describe the StashSet and 
%then show the query procedure.
%Formally, the StashSet is composed of the main stash and two identical ordered sets 
%containing $k \leq c$ temporary stashes. Since, the main 


The StashSet is structurally similar to the DR-LogSet and contains $k \leq c$ temporary stashes, organized in the {\em ascending} order of their Stash IDs. Analogous to the bigentry logs in the DR-LogSet, each temporary stashes (of fixed size) contains at least $c$ dummy blocks, in addition to the real blocks. The blocks are encrypted and randomly shuffled and a search index tracks the location of blocks. 

Each temporary stashes is periodically reshuffled (at least once every $c$ accesses) to ensure that unique dummy blocks are available for each access. As in case of the DR-LogSet, the reshuffled versions of the temporary stashes are written to a separate location on the server allocated for temporarily storing the reshuffled temporary stashes, namely the {\em  Reshuffled-StashStore}. The reshuffled temporary stashes in the Reshuffled-StashStore replace the old versions in the StashSet after $c$ queries. 
 
 \begin{small}
 	\begin{algorithm}
 		\caption{readStashSet($id$)}\label{readstashset}
 		\begin{algorithmic}[1]
 			\State // Acquire StashSet Lock
 			\State $i$: Read value of {\em StashSet Access Counter}
 			\If{$i = c$}
 			\State //Replace temporary stashes in the StashSet with their reshuffled versions in the {\em  Reshuffled-StashStore}
 			\State // Clear {\em  Reshuffled-StashStore}
 			\State $i = 0$
 			\EndIf
 			\State Stash Access Counter = $i + 1$.
 			\State // Release StashSet Lock
 			\For{$TempStash_{j} \in StashSet$}
 			\State $index\_blk$: Read index for $TempStash_{jj}$
 			\If {$id \in index\_blk$ and $id$ not already found}
 			\State Read $id$ from $TempStash_{j}$
 			\Else
 			\State Read $dummy$ from $TempStash_{j}$
 			\EndIf 
 			\EndFor
 			\State $TempStash_{i}$: Read $i^{th}$ temporary stash from the StashSet
 			\State $TempStash_{i}.reshuffle(rand)$
 			\State // Add $TempStash_{i}$ to the {\em  Reshuffled-StashStore}
 		\end{algorithmic}
 	\end{algorithm}
 \end{small}
 
 \noindent
 {\bf Querying the StashSet.~}
 % 
 The reshuffle is performed as part of the $\mathbf{readStashSet}$ (Algorithm \ref{readstashset}) that is also used to read the temporary stashes in Step 2 of the query protocol. To track the number of accesses to the StashSet, the server stores a {\em StashSet Access Counter (SAC)}, which is public information. This is accessed and updated by queries while holding a mutex, namely the {\em StashSet lock}.
 
  Specifically, the client first acquires the {\em StashSet lock} and reads the value of the SAC. If the value of the SAC is $c$ -- the StashSet has been accessed $c$ times since the temporary stashes were reshuffled -- the temporary stashes are replaced with their reshuffled versions in the {\em  Reshuffled-StashStore} and the SAC is reset. (Steps 3 - 6). The value of the SAC is incremented for each StashSet access (Step 7). The StashSet lock prevents ongoing parallel queries from accessing the StashSet while the temporary stashes are being replaced with their reshuffled versions. Note that this mechanism ensures minimal waits since reading and incrementing the SAC is inexpensive  and replacing the temporary stashes only involves copies between server-side data structures, {\em independent of network bandwidth}. 
 

%\smallskip
\noindent
%{\bf Querying the StashSet.~}
%
%The $readStashSet$ (Algorithm \ref{readstashset}) operation reads a block
%from the temporary stashes in descending order of the stash IDs.  All
%queries are to the read-only set.

Additionally, after releasing the StashSet lock, for each temporary stash, the client first reads its search index followed
by one block -- the required block (if present), or a unique (previously
un-accessed) dummy block (Steps 9 - 14).  As location of blocks in the temporary stashes
are randomized, reading a real data block is indistinguishable from reading
a dummy block. 

Finally, the client reshuffles the $i^{th}$ temporary stash from the StashSet where $i$ is the value of the SAC read by the client in Step 2. The reshuffled temporary stash is written to the {\em  Reshuffled-StashStore}.

Note that unlike the bigentry logs in the DR-LogSet, entries corresponding to blocks that are accessed from a temporary stash are not removed from the search index. Instead, dummy blocks are numbered (information stored in the search index) so that an access reads the $i^{th}$  dummy block from each temporary stash, where $i$ is the value of the SAC read in Step 2. This ensures unique dummy blocks are read by each access. 


%\todo{after reading the search index do we also remove the
%block ID from it and write the re-encrypted index back?}
%
%\todo{overall the stashset seems very similar to the log set structure in
%some sense -- is there a bigger lesson here? or maybe a unifying single type
%of structure for both?}

%Dummy blocks are 
%numbered so a unique dummy block can be accessed for each of the first $c$ queries. 
%
%After $c$ accesses, a temporary stash can run out of unique dummy blocks. 
%In this case, it needs to be reshuffled again before future accesses.  This
%is performed as part of the queries.  Specifically, each query reshuffles
%one temporary stash and uploads the new version to the update-only set.  The
%temporary stash reshuffled by a particular client is determined by the order
%of query execution.  Specifically, if the client registers the $i^{th}$ ($i
%\leq c$) entry to the query log (in Step 1 of the query protocol), it
%shuffles the $i^{th}$ temporary stash in the StashSet, when counted in the
%ascending order of the stash IDs.  This ensures that all temporary stashes
%in the StashSet are reshuffled every $c$ accesses \todo{``as well as the
%fact that no two clients interfere in reshuffling a given stash''? or
%similar }.  Once all the temporary
%stashes have been reshuffled (all queries with entries in the query log have
%finished execution), the update-only set becomes the read-only set and is
%used for future queries.
%	

\begin{customlemma}{2}
\label{stashset_lemma}
%
The accesses to the StashSet produce transcripts that are indistinguishable
and independent of the block that is being queried.
% 
\end{customlemma}
 
 Proof in Appendix.

\begin{figure}
	\includegraphics[scale=0.045]{figures/eviction_commit}
	\vspace{-0.3cm}
	\footnotesize{\caption{Eviction commit includes updating the
position map, updating the path on the data tree and adding the temporary
stash to the StashSet.}\label{eviction_commit}}
\end{figure}

\begin{small}
\begin{algorithm}
	\caption{$StashSet.add(TempStash_{i})$}\label{setstash}
	\begin{algorithmic}[1]
		\If{$StashSet.contains(TempStash_{i-1})$}
		\State // Replace $TempStash_{i-1}$ with $TempStash_{i}$
		\Else
		\State //Add $TempStash_{i}$
		\EndIf
	\end{algorithmic}
\end{algorithm}
\end{small}


%\smallskip
\noindent
{\bf Asynchronous commit.~}
%
The commit (Figure~\ref{eviction_commit}) incorporates three changes to
the protocol described in Section~\ref{oram:evict_background}.  

{\bf First}, the temporary
stash is added to the StashSet from the server-side cache (Algorithm \ref{setstash}).

{\bf Second}, instead of copying the entire eviction path from the W/O tree to the
data tree, only a part of the path may need to be updated based on the state
of commits.  This is because a subset of the EST buckets may have been
already updated by more recent evictions that accessed the critical section
later, but committed earlier.  These buckets are in their most recent state
and need not be updated during the commit.

These buckets can be identified based on the order in which evictions
executed the critical section.  In particular, while writing back the
metadata to the data tree during a commit (described next), the eviction
also stores a {\em timestamp} in the metadata for the EST buckets.  The
timestamp is the value of the {\em temporary eviction ID} of the eviction. 
When a future eviction commits, it checks whether the timestamp for the EST
buckets is ``later'' than its own timestamp, in which case it does not
overwrite them.  The rest of the eviction path (non-EST) buckets is copied
from the W/O tree to the data tree.

{\bf Third}, the metadata on the data tree path and the position map are updated
based on the current state of the bigentry log from which blocks are being
evicted to the data tree.  Specifically, the search index identifies blocks
that have been accessed by future queries (executed after the eviction had
started).  Recall that once a block has been accessed from a bigentry log,
the corresponding entry is removed from the search index.  The metadata and
position map entries for these blocks are not set by the commit as more
recent copies possibly exist in other log(s).  Consequently, the old copies
are inaccessible to queries and can be removed from the eviction path during
later evictions.

%\todo{all the above is simply too complex -- people will get lost. i don't
%have a solution other than to maybe summarize what we achieve by doing all
%that Firstly-Thirdly stuff.}

%%\smallskip
\noindent
{\bf Query Log.~}
%
The query log functions as described in Section \ref{oram:queries} with the
only difference being that a new query log is generated for each round of
queries, which is then cleared when the corresponding DRL is evicted to the
tree.  A client must read all such query logs  at the start of a query although only one will be active during the current query round. This is because the query log entries  
indicate to the client that the corresponding blocks will be found in the DR-LogSet and the queries to the data tre, PD-ORAM etc. should be fake accesses.
 %%\smallskip

\noindent
{\bf Correctness of evictions.~}
%
{\em None of the steps of the processing and the commit conflict with each other}. 
In particular, the processing only updates the W/O tree while the commit
updates the data tree.  During commits, the part of the path copied from the
W/O tree (non-EST buckets) to the data tree does not conflict with the path
that is updated in Stage 3 of the processing.

One invariant is that ongoing evictions only conflict for the EST buckets. 
Thus, processing and commits can safely execute in parallel as per the
transaction schedule (Figure~\ref{transact_sched}) while the processing locks enforce consistency for critical sections. 

We still need to show however that even with asynchronous commits, queries
can access the most recent version of a block at all times even when
evictions do not commit in the order of their assigned IDs:

\begin{customthm}{3}
\label{lemma:stashset}

% Even when evictions do not commit in the order of their 
% assigned IDs, the 
The most up to date version of a block is found either on the path indicated 
by the position map, in the StashSet or in the DR-LogSet.

\end{customthm}

Proof in Appendix.


\begin{small}
\begin{algorithm}
 \caption {client.Query(id)}\label{query}
 \begin{algorithmic}[1]
 \State // Acquire Query Lock, $L_{q}$
 \State Append entry to query log
  \State Read query lock
  \State // Release $L_{q}$	
  \State $i$ = $QueryLog.length\%c$ 
 \State $stash = readStashSet(id,i)$
 \State $leafID$ = PM.read(id)
 \State $path = DataTree.readBlocksFromPath(leafID)$
 \State // Request order based synchronization
 \State $BlocksFromLogSet = readLogSet(id)$
 \State $blk$ = Locate in $BlocksFromLogSet + path + stash $
 \State Update $blk$ for writes
 \State $writeLogSet(blk)$
 \end{algorithmic}
\end{algorithm}
\end{small}


% The eviction 
% clients 
% that have started after this eviction client reads the temporary stash while 
% evicting 
% to their respective path. Once the eviction commits, the temporary stash created 
% by the 
% eviction becomes the stash for the RingORAM data tree. 


\subsection{Query and Analysis} 
\label{oram:parallel_evict:analysis}


%\begin{figure}
%	\centering
%	\includegraphics[scale=0.15]{figures/query_parallel.eps}
%\end{figure}

 
Algorithm \ref{query} describes the modified query protocol.  The only
modification to the protocol in Section \ref{oram:queries} is that the
client additionally needs to query the DR-LogSet and the StashSet.
 
%The query protocol ensures that only a single updated copy of a block
%remains in the DR-LogSet at all times.  This is because a block that is
%queried from the DR-LogSet in Step 9, is appended to the DRL using
%$writeLogSet$ in Step 12.  Thus, if the block is found in any of the logs in
%Step 9, it is effectively deleted from that log by removing the entry from
%the search index (Algorithm \ref{readlogset}, Steps 7 and 10).
 
 
 
%%\smallskip
%\noindent
%{\bf Correctness of queries.~}
%% 
%Note that queries and the eviction processing do not overlap on access for
%any shared data structure and can therefore be executed concurrently as per
%the transaction schedule (Figure~\ref{transact_sched}).  Also, queries and
%commits are never executed in parallel since they require the
%query lock.  As shown by Lemma~\ref{lemma:stashset}, the most up to date
%%\todo{not ``the most updated''!! that means something else :)}
%version of any block will be found in either the data tree, the StashSet or
%the DR-LogSet, all of which are accessed by the query protocol.  Thus, the
%query is guaranteed to find the most updated copy of a block even if it is 
%being evicted in the background.
 
 

\begin{customthm}{4}
% 
With the modified query protocol (Algorithm \ref{query}) \sysname~ produces
indistinguishable access transcripts that are independent of the item being
accessed.
% 
\end{customthm}
  
Proof in Appendix.
 
 
%\smallskip
\noindent
{\bf Query Complexity.~}
%
In practice, the cost of queries increase for supporting parallel background
evictions.  This is a result of the additional blocks that need to be read
from the DR-LogSet
%\todo{DR-Logset? please be consistent everywhere once you
%name something. this is all over the place.} 
and the StashSet (bounded by the number of parallel
clients), and the cost of reshuffling logs and temporary stashes.  The
asymptotic complexity is still bounded by $\order{logN + c}$.


%\smallskip
\noindent
{\bf Eviction processing cost.~}
%
% The cost of processing can be evaluated in terms of the three 
% stages. 
% 
Stage 1 and Stage 3 are both $\order{log^{2}N}$ as they read and write back
$\order{logN}$ sized buckets along the path on the W/O tree (excluding the
small number of EST buckets).  These steps can be performed in
parallel without blocking queries and other ongoing evictions.

Only {\em one} eviction can execute in stage 2 at a time.  This includes
reading and writing back $\log{c}$ EST buckets and the temporary stash.  The
overall asymptotic complexity of this stage is $\order{logc \times logN}$. 
This is significantly less expensive than Stage 1 and 2 for
realistic deployment scenarios.  In fact, stage 2 becomes 
% prohibitively
expensive only when there are N parallel clients!


%\smallskip
\noindent
{\bf Eviction commit cost.~}
%
The eviction commit sets the metadata on the data tree path.  This has an
asymptotic complexity of $\order{logN}$, but the practical overhead is
negligible due to the small metadata size.  In addition, the commit copies
data between several server-side data structures (W/O tree, server-side
cache etc.) -- this adds negligible overhead since it does not impact
network bandwidth.  In effect, the eviction commits are significantly
cheaper than queries.




%\smallskip
\noindent
{\bf Bounding the DR-LogSet size.~}
%
%The number of logs currently in the DR-LogSet depends on the number of ongoing parallel evictions. 
%With queries executing independently of the evictions, this can potentially lead to an unbounded DR-LogSet.
%Therefore, it is necessary to enforce a mechanism which controls the rate 
%at which queries are executed with respect to the 
%rate of evictions. Fortunately, we only need to address the case where queries 
%are generated at a faster rate 
%since with slower queries, DRLs are generated and added to the 
%DR-LogSet at a rate slower than the rate at which they 
%are cleared by the evictions. 
% 
The transaction schedule (Figure~\ref{transact_sched}) ensures that a bigentry log
%\todo{which log? this is confusing} 
is cleared every time a new DRL is added to the DR-LogSet.  To enforce this,
before a query registers an entry to the query log in Step 1, it checks the size of the query log. 
If there are $c^{2}$ entries already in the query log ($c$ query logs with $c$ queries each), the query releases the {\em query lock} and waits for an eviction to complete.
%acquires the query lock (in Step 1 of the query protocol), it
%checks the size of the LogSet 
% In case, the LogSet is full, the query waits
%until an eviction commits and clears a log \todo{A DRL, a bigentry log ?!?} from the LogSet.



%It is worth noting here that due to unpredictable network delays and
%asynchrony, all parallel ORAM constructions without inter-client
%communication \cite{privatefs,taostore} provision for blocking
%queries\todo{what does provision for blocking queries mean?!?!} at
%some point of time to satisfy long outstanding requests.  For example, in
%TaoStore \cite{taostore}, a sequencer module running on the proxy ensures
%that queries are satisfied in the order that they are received.  This may
%result in a query waiting for a significant period of time before it
%receives a result due to network delays affecting previous results. 
%Similarly, PD-ORAM \cite{privatefs} uses a level progress monitor to ensure
%that queries and level reshuffles occur at similar rates, which may require
%slowing down queries.
%\todo{what was the purpose of this paragraph!?? summary/conclusion please}

%%\smallskip
\noindent
% 
{\bf Bounding the StashSet.~} Maintaining the transaction schedule bounds
the DR-LogSet but does not explicitly bound the StashSet.  This is because
the size of the DR-LogSet depends only on the number of eviction commits and
not on their order of execution.  For the StashSet the order of
commits is relevant.  

To see that the StashSet size is also bounded, first note that it
cannot contain both $TempStash_{i}$ and $TempStash_{i+1}$ for any given $i$
at the same time, as $TempStash_{i}$ would be overwritten with
$TempStash_{i+1}$ (Algorithm \ref{setstash}, Step 2).  Therefore, the only
scenario where the StashSet can contain $c$ stashes is when it contains
$TempStash_{p+i}, \forall i = 2j, 1 \leq j \leq c$, where $TempStash_{p}$ has the lowest Stash ID in the StashSet.

This corresponds to the case where $c-1$ evictions that started later,
finished execution and committed earlier than a currently ongoing eviction. 
In other words, if the longest running eviction started when the eviction
counter was $ctr$, now the eviction counter is at $ctr + 2c$.  Recall that
at this stage \sysname~ will not allow the eviction counter to increase
until the longest running eviction has committed.  This is an unlikely state
and is treated as a failed eviction.  In this case, the eviction is
reassigned to a new client and re-initiated.  In general, the effect of
possible network failure/system crashes and crash consistency for ORAMs is
orthogonal work and yet to be fully addressed in literature.

%
%\begin{figure}
%% \includegraphics[scale=0.06]{figures/eviction_parallel_new.eps}
% \includegraphics[width=8.5cm]{figures/eviction_parallel_new.eps}
% \vspace{-0.5cm}
% \caption{\footnotesize{The \sysname~ parallel eviction protocol. The client first 
% reads the DRL and the eviction path from the data tree (Steps 1 and 2). Then,
%it acquires a lock on the write-only tree and an eviction ID, $i$ from the controller. The client
%then reads the buckets on the eviction sub-tree (EST) from the 
%write-only tree and the temporary stash uploaded by the previous eviction, $TempStash_{i-1}$ (Steps 3 and 4).
%Next, a client-side merge creates the new path to be evicted and a temporary stash $TempStash_{i}$ (Step 5). The client writes back $TempStash_{i}$ and buckets on the EST to the 
%write-only tree (Steps 6 and 7). The client releases the lock on the write-only tree and writes back the complete eviction path to the write-only tree (Step 8). 
%Finally, the eviction commits after first blocking new queries temporarily to ensure a consistent state of the shared 
%data structures: the client uploads an updated 
%PM Result Log which will now form the PD-ORAM top level and the metadata for the eviction path
%into the data tree, the controller copies the eviction path from the write-only tree to the data tree and
%adds $TempStash_{i}$ to the StashSet. All logs corresponding to the eviction are cleared.}\label{evict_fig}}
%\end{figure}
%
%
%
%%%\smallskip
%\noindent
%{\bf Evictions.~}
%%
%The eviction protocol (Algorithm \ref{evict}, Figure \ref{evict_fig}) has significant changes from 
%Section \ref{oram:queries}. After reading the 
%current DRL and eviction path from the 
%data tree (Step 1 -2), the client waits to acquire a lock on the write-only tree (Step 3). 
%The eviction client is assigned an ID $i \leq k$ by the ORAM controller based on the value of a
%counter. More specifically, the client acquires the lock 
%only when eviction client $i-1$ releases the lock on the write only tree, as 
%enforced by the controller. 
%Note that the controller does not enforce an order in which the eviction clients can acquire locks -- 
%even if client $x$ starts evictions {\em after} one (or more) round of queries after client 
%$y$ started, client $x$ 
%is still granted the lock if it requests before client $y$. This is indeed possible 
%due to network delays -- client $y$ may require significantly more time to perform Steps 1 and 2 
%before requesting for the lock as compared to client $x$.
%
%Next, the client reads the temporary stash, $TempStash_{i-1}$ written by eviction client $i-1$ 
%and the buckets on the EST that intersect with the current eviction path (Step 5 and 6). Then, it 
%locally updates the buckets on the path read in Step 2 with the buckets read from the EST (Step 6). The 
%blocks from the DRL, the temporary stash and the blocks from the path are merged randomly 
%(Step 8). 
%
%The union of the blocks 
%created in Step 8 is evicted to a 
%new locally created path and a new temporary stash, $TempStash_{i}$ (Step 9 - 10). 
%The client writes back the temporary stash 
%and the buckets from the new path that 
%intersect the EST before releasing the lock (Step 11 - 15). 
%
%Once the client completes writing back to the write-only tree (Step 16), 
%it updates the position map. Before adding an entry to the position map, the client checks 
%the updated (current) index block for the log it is evicting from in order 
%to determine blocks that have been 
%removed from there while the eviction was in progress. Since, an updated copy of 
%these blocks necessarily exist in more recent logs, the client does not add an entry for these blocks 
%to the position map.
%This ensures that only the most updated copy of the block has an entry in the position map.
%The full path is copied from the write-only tree to the data tree (Step 17 - 21) and the client 
%updates the bucket-specific metadata on the data tree path. The metadata tracks only those 
%blocks that have the most recent version in the corresponding bucket 
%thus allowing future evictions to remove duplicates.
%
%Finally, the client indicates to the controller to add $TempStash_{i}$ in the StashSet.
%The controller adds the temporary stash to the StashSet while following 
%the protocol in Algorithm \ref{setstash} . Specifically, 
%$TempStash_{i}$ is set as the current stash only if all other stashes 
%$TempStash_{j}, j < i$ are present in the StashSet (Step 1 and 2). If not, 
%and the StashSet contains $TempStash_{i-1}$, then the controller replaces 
%$TempStash_{i-1}$ with $TempStash_{i}$ (Step 4 and 5). Otherwise, $TempStash_{i}$ 
%is added to the StashSet.
%
%The intuition behind this protocol is to maintain a consistent 
%set of temporary stashes while evictions commit asynchronously. Note that 
%the ID assigned to an eviction client is based on the order in which 
%it updates the shared data structures. Thus, if all eviction clients commit 
%synchronously similar to Section \ref{oram:queries}, 
%there will only be a single stash 
%as the temporary stash uploaded by a client will always be the current stash. 
%Otherwise, suppose eviction client $i$ commits before 
%eviction client $i-1$. In this case, the protocol ensures that 
%$TempStash_{i}$ is added without overwriting any previous temporary 
%stashes already in the StashSet, thus preserving the existing consistent 
%state of the StashSet. On the other, if client $i$ commits after $i-1$, 
%$TempStash_{i-1}$ can be overwritten with $TempStash_{i}$ as the most updated version of 
%$TempStash_{i-1}$ has already been used for eviction by client $i$. Thus, the 
%blocks in $TempStash_{i-1}$ are either on the path evicted to by client $i$ or 
%in $TempStash_{i}$. We formally 
%prove the correctness of the protocol below.
%
%Note that the eviction protocol blocks new queries for a brief period of time when 
%the position map is updated (the top level of PD-ORAM is created), 
%the path is copied to the data, 
%the metadata is added to the data tree path to the data tree and the temporary stash 
%is added to the StashSet. Further, the corresponding log from 
%the DR-LogSet is cleared after all queries with entries in the current query log 
%have completed accesses to the DR-LogSet (Steps 8 - 13, Algorithm \ref{query}). 
%This ensures a consistent view of the DR-LogSet for already executing queries.
%The time required to complete all steps of the eviction commit
%is significantly small compared to the 
%time required to read and write back the path from the tree for the eviction. 
%Also, as most cloud services (such as Amazon AWS) already support 
%copy operations, copying the path from the write only tree to the data tree does 
%not require additional client communication and thus is not affected by network 
%latency.
%
%
%
%
%
%
%%%\smallskip
%\noindent
%{\bf Correctness.~}
%%
%As discussed before, the eviction procedure can be divided into four main steps -- i) reading the path for eviction, ii) reading the buckets from the EST and the 
%previous temporary stash and uploading the updated EST buckets and a new temporary stash, 
%iii) writing back the path and iv) updating the position map and setting the temporary 
%stash in the StashSet. Out of these steps, i) and iii) can be performed without violating consistency as they do not update/write to 
%any buckets that overlap with other evictions. The buckets on the EST (intersecting with other parallel evictions) are updated with a lock to 
%ensure consistency of the write-only tree. Further, the eviction considers the most updated version of the 
%stash uploaded 
%by the 
%previous eviction clients and uploads an updated temporary stash to be used by the next eviction client. 
%Consequently, these steps establish a 
%non-overlapping and consistent order of accesses to the shared data structures.
%
%Step iv) however requires closer scrutiny. This is because 
%even though eviction client $i$ acquires lock and updates the data structures before eviction client $i+1$ in Steps 3 - 15, and 
%the outcome of the eviction for client $i+1$ depends on these updates, client $i+1$ 
%can commit asynchronously before $i$ . We show below
%that consistency of the shared data structures is maintained even in this case.
%
%
%\begin{customthm}{3}
% The parallel eviction protocol ensures that even when evictions do not commit in the order of their 
% assigned IDs, the most updated version of a block is found either on the path indicated 
% by the position map, in the StashSet or in the DR-LogSet.
%\end{customthm}
%
%Proof in Appendix.
%% \begin{proof}
%%  First, consider the case where client $i+1$ commits before client $i$. In this case, $TempStash_{i+1}$ has to be inserted into the 
%%  StashSet before $TempStash_{i}$. Naively setting $TempStash{i+1}$ as the current stash obviously violates consistency since the 
%%  blocks that belonged to all previous stashes will be overwritten. 
%%  
%%  Also, consider a block $x \in TempStash_{i}$. $TempStash{i}$ was created considering the blocks from $TempStash{i-i}$, a path 
%%  $p$ from the data tree and the corresponding log, $l$ in the LogSet. Thus, there are the following three cases that are possible: $x \in TempStash_{i-1}$,
%% $x \in p$ and $x  \in l$. As $l$ and $p$ are unmodified as $i$ has not committed and $TempStash{i-1}$ is in the StashSet, a client querying for 
%% $x$ will find the block in one of the three locations. Thus, $TempStash_{i+1}$ is added to the StashSet without overwriting previous stashes (Step 7).
%% 
%% Now consider the case, where $i$ commits before $i+1$. In this case, for $x \in TempStash_{i}$, then $x$ was also considered in the union evicted to path $p^{i}$ 
%% in step 9. Thus, now $x \in p^{'}$ after the path has been updated, 
%% or $x \in TempStash{i+1}$. Thus, over writing $TempStash_{i}$ with $TempStash_{i}$ (Step 5) does not violate consistency.
%% 
%% Finally, if all evictions committed in the order of their ID, the current stash would be the temporary stash uploaded by the recently committed eviction.
%% This is because the ID is assigned based on the order in which the client update the shared data structures and these modification are 
%% considered for successive evictions. This corresponds to the case where $StashTemo_{i}$ is set as the current stash (Step 2).
%%  
%% \end{proof}
%
%
%%%\smallskip
%\noindent
%{\bf Bounding the DR-LogSet size.~}
%%
%The number of logs currently in the DR-LogSet depends on the number of ongoing parallel evictions. 
%With queries executing independently of the evictions, this can potentially lead to an unbounded DR-LogSet.
%Therefore, it is necessary to enforce a mechanism which controls the rate 
%at which queries are executed with respect to the 
%rate of evictions. Fortunately, we need to address only the case where queries 
%are generated at a faster rate than the evictions 
%since with slower queries, DRLs are generated and added to the 
%DR-LogSet at a rate slower than the rate at which they 
%are cleared by the evictions. 
%
%\sysname~ employs a simple mechanism to achieve this by allowing 
%the controller to block a new round of queries once the DR-LogSet
%is full, until an eviction commits. Specifically, for a round of queries 
%that begins at time $t_{1}$ (determined 
%from the first access to a new query log) and ends at time $t_{2}$ (determined from the $c^{th}$ 
%block appended to the current DRL), if no ongoing eviction commits between $t_{1}$ and $t_{2}$, 
%the controller blocks new queries until an eviction commits. Note that this corresponds to the 
%case where an eviction requires more than $c$ rounds of queries in between to complete. 
%Blocking the queries
%ensures that a new log is added to the DR-LogSet only when a previously added log is cleared. 
%Fortunately, emperical results show that this is an unlikely case, since even with 
%purely synchronous queries and evictions, the time required for performing an eviction 
%after $c$ queries is roughly equal to the total time required to perform the $c$ queries \cite{ringoram}.
%
%It is worth noting here that due to unpredictable network delays and asynchrony, all previous parallel 
%ORAM constructions without inter-client communication provision for blocking queries at some point of time 
%to satisfy long outstanding requests. For example, in TaoStore \cite{taostore}, a sequencer 
%module running on the proxy ensures that queries are satisfied in the 
%order that they are received. This may result in a query waiting for a significant 
%period of time before it receives a result due to network delays affecting previous 
%results. Similarly, PD-ORAM \cite{privatefs} uses a level progress monitor to ensure that 
%queries and level reshuffles occur at similar rates which may require slowing down queries, 
%as discussed before.
%
%%%\smallskip
%\noindent
%{\bf Bounding the StashSet.~} Bounding the DR-LogSet using the mechanism described above does not 
%bound the StashSet. This is because the size of the DR-LogSet depends 
%only on the number of eviction commits and not on the order in which the commits take place.
%However, for the StashSet the order of commits is relevant.
%To bound the StashSet, first
%note that the StashSet cannot contain both $TempStash_{i}$ and $TempStash_{i+1}$ for 
%any given $i$ at the same time, 
%as $TempStash_{i}$ would be overwritten with $TempStash_{i+1}$ (Algorithm \ref{setstash}, Step 5). 
%Also, if the StashSet contains $TempStash_{1}$, that would 
%be set as the current stash (Algorithm \ref{setstash}, Step 2). 
%Therefore, the only scenario where the StashSet can 
%contain $c$ stashes is when it contains $TempStash_{i}, i = 2j,  1 \leq j \leq c/2$. 
%This corresponds to the case where 
%eviction client with ID 1 has not 
%committed even when client with ID $c$ has committed. In other words, $c$ rounds of queries (and at least 
%one eviction) has been performed 
%since client 1 started eviction. Note that such a state is unlikely if all clients have similar bounded 
%network 
%latencies. However, in such cases the controller blocks the queries to allow 
%eviction client 1 to finish.
%
%
%%%\smallskip
%\noindent
%{\bf Query Complexity.~}
%%
%The construction presented here features a higher practical 
%query complexity as compared to the construction in Section \ref{oram:queries}
%since a block has to be read from each of the additional logs 
%in the DR-LogSet and the StashSet. Also, the size of the query log increases by a 
%factor of $\order{c}$ as $c$ previous DRLs may be undergoing 
%evictions at a time. Note that since we ensure that the DR-LogSet and StashSet size, $k < c$, 
%the overall asymptotic complexity is still $\order{logN + c}$. 
% 
%
%
%
%
%
%


==> parallelqueries.tex <==
\section{Parallel Queries}
\label{oram:queries}

The first step towards providing full parallelism is performing ORAM queries in parallel. 
Privatefs~\cite{privatefs} shows how any ``non-simultaneous'' ORAM\footnote{Applicable for any ORAM that is designed for deployment on standard storage devices where physical sectors are accessed serially} 
can be converted to an ORAM with support for parallel queries. Unfortunately, for tree-based ORAMs, this is not enough since the main performance bottleneck is the expensive eviction 
step.

In the following, we  first describe a parallel query mechanism for \sysname~. Then in Section \ref{oram:evictions}, we introduce a novel parallel eviction protocol, enabling \sysname~ to reap the full benefits of parallel accesses.

\noindent
{\bf Data tree.~}
% 
\sysname~ organizes data blocks in a server-side binary data tree, similar in format
to a RingORAM tree~\cite{ringoram}. Specifically, each node of the 
tree is a bucket containing a fixed number of data blocks and dummy blocks, 
encrypted with semantic security and 
randomly shuffled. Each bucket also stores relevant 
metadata for retrieving specific data blocks, identifying dummy 
blocks etc.
 
A fixed-sized stash for the data tree is stored on the server. Empirical 
bounds~\cite{ringoram} on the stash size ensure that overflows are negligible
with very high probability.


One of the main challenges of achieving
concurrency for position map based ORAMs is due to the position map entries
being stored recursively (on remote storage) in smaller ORAMs.  More
specifically, the position map for the data ORAM is stored in a separate
smaller ORAM on the server, the position map of which is stored in yet another smaller ORAM. 
The number of entries per position map block determines the number of levels
of recursion.  Since each position map block contains more than one entry,
concurrent access by two or more clients to the same position map block
allows the server to correlate these accesses.

%\smallskip
\noindent
{\bf PD-ORAM.~}
% 
\sysname~ solves this by storing the position map entries in a separate
PD-ORAM \cite{privatefs} instance on the server, indexed by logical block ID
and containing the corresponding leaf ID in the data tree to which the
data block is mapped.  PD-ORAM is used to ensure that clients
can access individual position map entries directly. By construction PD-ORAM supports parallel queries
without leaking correlations between concurrently accessed items. 


% 
% Since each level of PD-ORAM contains multiple fixed-sized buckets,
% an entry for a particular logical block ID, if it exists in a PD-ORAM level,
% is located in the bucket determined by applying the secret hash function for
% that level on the logical block ID.  Clients query for a position map item
% by downloading the corresponding bucket from each level of PD-ORAM as
% determined by the hash function for that level.  If the entry is found at a
% particular level, the client downloads random buckets from each of the
% subsequent levels.

%\smallskip

In addition, \sysname~ makes use of a number of append-only logs to synchronize client accesses
without direct communication.
% used by the clients to
%synchronize  
%\smallskip

\noindent
{\bf Query log.~}
%
A query log records all currently ongoing transactions.  Clients append the
logical ID of the data block they are querying for and download the query
log to check for overlapping accesses.  In case of an overlapping query -- there is a previous entry for the same block in the
query log -- the client proceeds with a dummy access (described
later).  The query log ensures that all clients have a consistent view of
ongoing transactions.

%\smallskip
%\noindent
%{\bf PM result log.~}
%%
%The PM result log contains items that have already been accessed since the
%last eviction from the position map.  After reading an entry from the
%position map, a client re-encrypts and appends the entry to the log. 
%Similar to \cite{privatefs}, the entries in the PM result log form the top
%level of PD-ORAM \cite{privatefs}.

%\smallskip
\noindent
{\bf Data result log (DRL).~}
%
The DRL contains data blocks that have been accessed since
the last eviction. The DRL effectively caches previously accessed blocks until an ORAM eviction places them back to random locations on the data tree.

\noindent
{\bf Query lock.~}
%
\sysname~ uses a mutex, namely the {\em query lock} to access the query log. The lock is held for only short periods of time as described later.


%two fine-grained locks for accesses to the append-only logs -- clients access the query log after acquiring the {\em query lock}, $L_q$, and similarly the DRL is accessed after acquiring the {\em result lock}, $L_r$. 
\begin{figure}
\centering
\includegraphics[scale=0.18]{figures/query_serial}
\vspace{-0.5cm}
\footnotesize{\caption{
%
Query overview.  Accesses to the stash, the position map (PD-ORAM) and the data tree can proceed concurrently. Queries access 
the query log after acquiring the query lock for a short period of time. Synchronizing accesses to the DRL is required to ensure that queries are completed in the order in which they start execution, a necessary condition to prevent security leaks (Section~\ref{model}). \label{query_overview}}
%
}
\end{figure}


A client query includes the following steps that are executed in order (Figure \ref{query_overview}):

\begin{enumerate}

\item The client acquires the {\em query lock}. Then, it appends the required logical block ID to the query log and downloads the entire query log. The query lock is released.

\item The client downloads the entire stash from the server.
 
\item  If the required block is already being accessed by
another client (determined from Step 1), or the block has already been found in the stash in Step 2, the client perfoms a {\em dummy access} by reading random
buckets from PD-ORAM. Otherwise, the client queries the position map PD-ORAM \cite{privatefs} 
for the leaf ID corresponding to the required logical block ID. 


\item In case the access to PD-ORAM in Step 3 was a dummy access, the client reads {\em only} dummy
blocks from a randomly selected path of the data tree. Otherwise, the client reads metadata from the data tree along the path on which the required block exists (as determined from the
position map entry in Step 3).  Based on the metadata, a block is read from each 
of the buckets -- the required block (if present), or a dummy block.

\item {\bf Request order based synchronization:} The client waits for ``previous'' clients to finish their queries. 
Specifically, queries that started execution earlier by registering an entry in the query log in Step 1, must complete {\em all} steps of the query protocol before the client can proceed. The client checks this by comparing the size of the current DRL and the ordering of entries in the query log. If the client registered the $i^{th}$ entry to the query log, it can proceed only after there are $i-1$ blocks in the DRL.

\item The client reads the DRL. In case of overlapping accesses, 
the up-to-date version of the required block will be found in the DRL. 

\item The client updates (for write accesses), reencrypts and appends the 
queried block to the DRL.

% If a client found the queried block in step 7, the client writes back
% the updated value of the block to the DRL for a write access.  Otherwise,
% the client re-encrypts and writes back the queried block found in Step 2 or
% Step 5.

\end{enumerate}

Note that in step 6, a client is guaranteed to find the most recent version
of the queried block after all previous ongoing transactions accessing the
block have completed.

% \begin{figure}
%  \includegraphics[scale=0.35]{figures/eviction.eps}
% % \vspace{-1cm}
%  \caption{High level description of the eviction process. Eviction steps, data items and locations, are randomized and independent 
%  of the client queries or data values.\label{eviction_fig}}
% \end{figure}


%\smallskip
\noindent
{\bf Eviction.~}
After a fixed number of accesses, the logs are cleared through an eviction
into the data tree. Queries are blocked during this period. The client that executes the last query before an eviction, proceeds with the 
following steps:

\begin{enumerate}

\item The client reads a
predetermined path from the data tree.

\item The client assigns random leaf IDs to each of the blocks in the DRL
and creates new corresponding position map entries which are inserted into
PD-ORAM (forming the new top level of PD-ORAM).

\item The client then merges the stash and the DRL (already read as part of the query) and evicts as many blocks
as possible along the path.

\item The client forms the new stash using the blocks (re-encrypted) that
could not be evicted back to the tree from the combined DRL and stash, and uploads it to the
server.

\item All logs are cleared.

\end{enumerate}

Since there may be multiple versions of the same block in the DRL 
due to concurrent accesses for the same block, only the latest
version is considered for eviction and all other copies are discarded.
To prevent the server from identifying duplicates
(which implies that two previous concurrent accesses queried for the same
block), the client adds fake position map entries corresponding to the
duplicate blocks.  This ensures that the number of entries
added to PD-ORAM during evictions is always equal to the maximum size of the DRL.

%\smallskip
\noindent
{\bf Efficiency and correctness.~}
% 
The protocol employs the {\em query lock} only for accessing the query log. The query log  contains several entries of $\log{N}$ bits and is expected to be small in size (e.g., 
the size of a data block for $\order{\log{N}}$ concurrent clients). Thus, registering an entry while holding the lock results in negligible wait times for other clients. 

For accessing the DRL in Step 6, a client must wait for previous clients to finish performing their queries. Since the most expensive steps of the protocol i.e., accesses to PD-ORAM, the stash and the data tree are performed in parallel, 
the wait time is not expected to be significantly long. 

Ordering accesses to the DRL ensures that logical requests are satisfied in the 
order in which they are received. 
As described in Section \ref{model}, this is necessary to ensure
query privacy for any ``non-simultaneous'' ORAM
which allows only serial execution of queries for the same underlying block\footnote{It may be noted that PD-ORAM~\cite{privatefs} employs a similar idea to ensure that queries are answered in the order in which they are received.}.


\begin{thm}
	\sysname~ produces indistinguishable access transcripts that are independent 
	of the item being accessed. 
\end{thm}

%\todo{this needs rewriting}

Proof in Appendix.


\subsection{Analysis}

Synchronizing on accesses to PD-ORAM (for storing position map entries) and the data tree is critical for security and
performance.  We now discuss parameters that impact
this.

%\smallskip
\noindent
{\bf Eviction Period.~} 
%
The ``eviction period'', $c$ determines the number of concurrent accesses
that can be performed before an eviction needs to occur.  Intuitively,
setting a higher eviction period increases parallelism but also incurs higher overheads 
due to increase in the DRL and query log size. \cite{ringoram} provides empirical bounds for the stash size as a function of the bucket size and the
eviction period.  \sysname~ uses these results to
determine a suitable eviction period for appropriately bounding the stash size.

% \smallskip
% \noindent
% {\bf Stash Size.~}
% %
% \sysname~ ensures that the stash always contains the same number of entries 
% irrespective of the 
% outcome of an eviction. More specifically, if the number of blocks in the stash 
% after an eviction is 
% less than the total size of the stash, \sysname~ adds fake blocks to the empty 
% locations.


%\smallskip
\noindent
{\bf PD-ORAM Bucket Size.~} 
% 
Recall that after an eviction, an entry is added to the PD-ORAM top level 
for each block in the DRL. Consequently, the top level should hold at least as
many entries as the DRL.  In \sysname~, the size of the top level
is equal to the eviction period, $c$.  To handle hash
collisions \cite{privatefs}, each bucket in the following levels contains
$c$ real entries and a number of additional fake entries up to a
total bucket size of $c \times logN$.

%\smallskip
\noindent
{\bf Query overhead for position map entry.~}
%
The size of a PD-ORAM bucket with $c \times logN$ position map entries,
with each map entry of size $\order{logN}$ bits, is roughly equal to the size of
a data block.  For a 1TB database, with 20 clients and 8 byte
position map entries, the size of a bucket is 4KB.  Thus, the
bandwidth overhead for a PD-ORAM query is equivalent to reading $\order{logN}$ data blocks of 4KB each.

The amortized bandwidth required for the reshuffle in PD-ORAM is $\order{log^{2}N}$ 
position map entries, or $\order{log^{3}N}$ bits since 
each position map entry is $\order{logN}$ bits.
With $\Omega(log^{2}N)$ sized 
data blocks (a common assumption 
for ORAMs proposed since \cite{pathoram}),
the amortized bandwidth for the shuffle is equal 
to $\order{logN}$ data blocks. Since, in PD-ORAM all level reshuffles are
performed in the background without stopping
queries, the additional bandwidth for each query due to the reshuffle is
upper-bound by $\order{logN}$.

The bandwidth overhead for storing the position map recursively using non-uniform block sizes (\cite{pathoram}) is also $\order{logN}$. Therefore, deploying PD-ORAM for storing the position map does not affect the overall bandwidth required for accessing data blocks
from the data tree, a critical fact.
% 

%For storing the position map recursively on the server, Stefanov {\em et
%al.}  show how to parameterize the recursion using
%non-uniform (smaller) blocks sizes for the position map ORAMs to achieve a
%bandwidth overhead of $\order{logN}$ data blocks to read a position map
%entry for a block.  
%%  to the performance of \sysname~.

%\smallskip
\noindent
{\bf Query complexity.~}
%
For a \sysname~ query, a client reads the stash, and a block from each of
the $logN$ buckets on a particular path on the data tree.  This has an
overall access complexity of $\order{logN}$.  Additionally, the client needs
to read the DRL and the query log, both $\order{c}$ in size.  Thus, the
overall access complexity for \sysname~ is $\order{logN + c}$.


% Note that although the query log 
% (which the client needs to read at the 
% start of the query) is $\order{c}$ in size, it barely affects the 
% overall practical bandwidth overhead, since each of the constituent entries of the query log
% is only a few bytes in size. 
% More specifically, with position map entries of $\order{logN}$ bits, the total size of 
% the query log is $\order{clogN}$ bits. With $\Omega(log^{2}N)$ sized data blocks, reading 
% the query log requires the same bandwidth as reading a data block with $c = \order{logN}$. 

% \todo{you have to decide if you
% treat $c$ as a constant or as a variable -- above you say ``$\order{c}$ in
% size'' and here you say this is a constant? or am i missing something?}. . 

% \smallskip
% \noindent
% {\bf Eviction complexity.~}
% %
% For an eviction, the evicting client reads the append logs, the stash and all the buckets 
% along a path on the tree.The append logs are bound by $\order{e} \in \order{logN}$ as shown 
% before while the stash is $\order{logN}$ in size. The main overhead for the 
% eviction is due to reading the buckets along the path where the bucket size, $z \in \order{logN}$. 
% In this case, the complexity of reading the path is $\order{log^{2}N}$. Since 
% the eviction is performed every $c = \order{logN}$ accesses, the amortized eviction 
% complexity is $\order{logN}$.



% \begin{proof}
% Consider two clients $c_1$ and $c_2$ that query for blocks $b_1$ and $b_2$ respectively. 
% If $c_1$ starts exection before $c_2$, the query log is updated by $c_1$ before $c_2$ can access it. 
% This allows $c_2$ to identify the block being accessed by $c_1$. 
% 
% If $b_1 \neq b_2$, the two queries can execute independently 
% as they access unrelated items.  
% The query includes appending 
% an encrypted item to each of the append-only logs and a query to PD-ORAM and 
% the RingORAM data tree. The state of the 
% logs (after appending an item) depends only 
% on the {\em number} of previous accesses (public information) 
% ,independent of the item being added. Also, the queries to PD-ORAM and the RingORAM data tree
% produce ``randomized transcripts'' as result 
% of their query privacy mechanisms.  Finally, $c_2$ waits for $c_1$ to 
% complete executing and appending a data block to the DRL
% before reading and appending $b_2$ (updated for writes) to the DRL.
% Due to semantic security, the two blocks added to the DRL are indistinguishable. 
% 
% Now, if $b_1 = b_2$, $c_2$ must wait for $c_1$ to finish execution 
% before it can access $b_1$, without leaking this information to the server.
% $c_2$ identifies that $b_1$ is already being 
% accessed by $c_1$ from the query log in Step 1. Then, 
% $c_2$ proceeds with a dummy query to PD-ORAM and the RingORAM data tree, 
% which produces transcripts indistinguishable from a real query. 
% An encrypted dummy item, indistinguishable from a real item is
% added to the the PM Result Log. Finally, $c_2$ finds $b_1$ in the DRL after $c_1$ completes executing 
% and writes back $b_1$ (updated for writes) to the DRL. As shown above, 
% even when $b_1 \neq b_2$, $c_2$ waits for $c_1$ to write back $b_1$ to the DRL before 
% it reads and appends $b_2$ (indistinguishable from $b_1$) to the DRL. This ensures identical transcripts for the two cases.
% 
% 
%  
% \end{proof}


% \begin{thm}
% %
% The existence of an adversary with a non-negligible advantage in violating
% query privacy (as defined in \cite{goldreich}) for \sysname~ implies the
% existence of an adversary with non-negligible advantage in violating query
% privacy for PD-ORAM (``query privacy inheritance'').
% %
% \end{thm}
% 
% % \smallskip
% \begin{proof}
% % \proofsketch
% % 
% First, note that all \sysname~ queries look identical to the server and are
% composed of the steps described above.
% 
% In effect, the server sees a transcript composed of a number 
% of reads/writes on semantically secure encrypted data at fixed public and 
% randomized locations (''randomized transcript") plus a PD-ORAM query.
%  
% Next, note that, if a client queries for a block that is being
% simultaneously accessed by another client, it issues a fake query which is
% indistinguishable from a real query.  Further, the server-enforced
% synchronization, ensuring that clients waiting for simultaneous accesses to
% finish accessing the queried block can obtain the most updated version of
% the block from the DRL, is based on public knowledge -- the
% order in which client connects (and appends entries to the query log).
%  
% Finally, consider an adversary $\mathcal{A}$ with non-negligible advantage
% in violating query privacy for \sysname~.  An adversary $\mathcal{B}$
% endowed with an equivalent advantage at violating query privacy for PD-ORAM
% can be then constructed as follows: $\mathcal{B}$ simulates $\mathcal{A}$
% for every query by appending random information to the append logs.  Since
% the entries in the logs, the blocks read from the data tree and the
% stash are encrypted with semantic security, any additional advantage to
% $\mathcal{A}$ by observing these entries/blocks read from the path implies a
% non-negligible advantage for $\mathcal{A}$ in distinguishing between the
% output of the semantically secure encryption and random. Effectively, the
% "randomized transcript" does not offer any non-negligible advantage.
% $\mathcal{B}$ then outputs the guesses and requests provided by
% $\mathcal{A}$, and obtains the same advantage as $\mathcal{A}$ (i.e., in the
% query privacy game of \cite{goldreich}).
% 
% %
% \end{proof}


% \begin{small}
% \begin{table*}
% \centering
%     \begin{tabular}{ | l | l | l | l | l | l | l |}
%     
%     \hline
%     
%     ORAM & Online (Query) Cost & Offline (Reshuffle) Cost & Client Communication Cost & Client Storage & Server Storage & Assumptions \\ 
% \hline
%       TaoStore \cite{taostore}  & $\order{logN}$ & $\order{logN}$ & N/A & $\order{NlogN}$ & $\order{N}$ & Trusted Proxy\\
%       Privatefs \cite{privatefs} & $\order{logN}$ & $\order{log^{2}N}$ & N/A & $\order{\sqrt{N}logN}$ & $\order{NlogN}$ & N/A \\
%       OPRAM \cite{chenpram} & $\order{log^{2}N}$ & $\order{logN}$ & $\order{logc \times logN}$ & $\order{logN}$ & $\order{N}$ & Client Interaction	\\
%       \sysname~	& $\order{logN + e}$ & $\order{logN + e}$ & N/A & $\order{\sqrt{N}logN}$ & $\order{NlogN}$ & N/a\\
%       \hline
%     \end{tabular}
%     
%     \caption{Asymptotic comparison of \sysname~ with other parallel ORAM constructions. Here, $e$ represents the eviction period for \sysname~ while $c$ represents 
%     the number of parallel clients in the case of OPRAM \cite{chenpram}.\label{asym_compare}}
% \end{table*}
% \end{small}

% \smallskip
% \noindent
% {\bf Asymptotic comparison with existing work.~}
% %
% Table \ref{asym_compare} compares \sysname~ with existing parallel ORAM constructions. Note that OPRAM \cite{chenpram} 
% and PrivateFS \cite{privatefs} have higher overall asymptotic overheads. TaoStore \cite{taostore} requires 
% higher client side storage to store the position map while {\em also operating under different assumptions and 
% requiring the addition of a trusted proxy in-between.}


